Identifying and Quantifying Trade-offs in Multi-Stakeholder Risk Evaluation with Applications to the Data Protection Impact Assessment of the GDPR

Cybersecurity risk management consists of several steps including the selection of appropriate controls to minimize risks. This is a difficult task that requires to search through all possible subsets of a set of available controls and identify those that minimize the risks of all stakeholders. Since stakeholders may have different perceptions of the risks (especially when considering the impact of threats), conflicting goals may arise that require to find the best possible trade-offs among the various needs. In this work, we propose a quantitative and (semi)automated approach to solve this problem based on the well-known notion of Pareto optimality. For validation, we show how a prototype tool based on our approach can assist in the Data Protection Impact Assessment mandated by the General Data Protection Regulation on a simplified but realistic use case scenario. We also evaluate the scalability of the approach by conducting an experimental evaluation with the prototype with encouraging results.

==> Removed/Algorithms.tex <==
\algnewcommand\algorithmicforeach{\textbf{for each}}
\algdef{S}[FOR]{ForEach}[1]{\algorithmicforeach\ #1\ \algorithmicdo}
% \begin{spacing}{1.125}
\begin{algorithm} \caption{Multi-Stakeholder Risk Assessment}
\begin{algorithmic}[1]
\small 
% \setstretch{1.25}
\State Input data:  List of Threats $\mathcal T$, Controls $\mathcal C$ and Protection Goals $\mathcal G$.
\State $Assumption~1$: For each threat, subset $\mathcal {C_T}$ and the compromised goals are identified. 
\State $Assumption~2$: Stakeholders $\mathcal S$ and their Preferences $\mathcal P$ are determined.
\State $N=0$;~~ Total number of compromised goals by threats
\ForEach {$t \in \mathcal T $}
$Q_{t}$=0;~~Number of compromised goals by $t$
\ForEach {$g \in \mathcal G $}
\If{$t$ compromises $g$}
\State $Q_{t}++$;
\State $N++$;
\EndIf
\EndFor
\EndFor
\ForEach {$t \in \mathcal T $}
\State $OW_t$= $\frac{Q_t}{N}$
\EndFor ~~~~~~~~~~~ \textit{$/_*$ Output: Observation Weights (OW) $_*/$}
% \State \textit{Output: Observation Weights (OW)}
\ForEach{$t \in \mathcal T $}
\State $sum=0$;
\ForEach {$c \in \mathcal C_T $}

\State $sum+=ml_c$;~~Assign a mitigation level ($ml$) to each $c$ $\gets \{0,0.5,1\}$
\EndFor
\State $TE_t=1- \frac{sum}{\mathcal {C_T}}$,~~ Where $0< TE_t \leq1$

\EndFor ~~~~~~~~~~~\textit{$/_*$ Output: Threat Existences (TE) $_*/$}
% \State \textit{Output: Threat Existences (TE) }
\State $sumTC=0$;
\ForEach{$t \in \mathcal T $}
\State $TC_t$= $TE_t \times OW_t$;
\State $sumTC += TC_t$;
\EndFor
\ForEach{$t \in \mathcal T $}
\State $NTC_t$= $\frac{TC_t}{sumTC}$
\EndFor ~~~~~~~~~~~\textit{$/_*$ Output: Normalized Threat Criticalities (NTC) $_*/$}
% \State \textit{Output: Threat Criticalities (TC) }
\ForEach {$s \in \mathcal S $}
\ForEach {$p \in \mathcal P $}
\State $APW^{sp}$  
\EndFor
\EndFor ~~~~~~~~~~~\textit{$/_*$ Output: Assigned Preference Weights (AWP) $_*/$}
\ForEach{$t \in \mathcal T $}
\ForEach {$s \in \mathcal S $}
\ForEach {$p \in \mathcal P $}
\State $IV^{sp}_t$  $\gets \{0,1,2,3,4\}$;~~Assign an impact value to each $p$ for each $t$ 
\EndFor
\EndFor
\EndFor ~~~~~~~~~~~\textit{$/_*$ Output: Impact Values (IV) $_*/$}
\ForEach{$t \in \mathcal T $}
\ForEach {$s \in \mathcal S $}
\ForEach {$p \in \mathcal P $}
\State $IL^s_t$ = $\Sigma ~~(IV^{sp}_t \times APW^{sp})$;
\EndFor

\algstore{bkbreak}
\end{algorithmic}
\end{algorithm}

% \end{spacing}
% And we need to put some additional text between\dots
\begin{algorithm}[]
\ContinuedFloat
\caption{Part 2}
\begin{algorithmic}[1]
\algrestore{bkbreak}
\small
\EndFor
\EndFor ~~~~~~~~~~~\textit{$/_*$ Output: Impact Levels (IL) $_*/$}
\ForEach {$g \in \mathcal G $}
\ForEach {$s \in \mathcal S $}
\State $sumRisk=0$;
\ForEach{$t \in \mathcal T $}
\If{$t$ compromises $g$}
\State $sumRisk += (NTC_t  \times  IL^s_t)$;
\EndIf
\EndFor
\State $GoalRA^s_g = sumRisk$;
\EndFor
\EndFor ~~~~~~~~~~~\textit{$/_*$ Output: Goal Risk Exposure for each Stakeholder $_*/$}

\ForEach {$s \in \mathcal S $}
\State $sum=0$;
\ForEach {$g \in \mathcal G $}
\State $sum += GoalRA^s_g$;
\EndFor
\State $FinalRisk^s = sum$;
\EndFor ~~~~~~~~~~~\textit{$/_*$ Output: Final Risk Exposure for each Stakeholder $_*/$}
\end{algorithmic}
\end{algorithm}


==> Removed/Background.tex <==
\section{Background}
\label{sec:Back}
We present some background notions required to define context, problem, and solution. 
%\subsection{\textbf{GDPR Concepts}}
%Regarding the process of personal data, General Data Protection Regulation (GDPR) was introduced to reinforce and standardize data protection. 
%The GDPR calls, in order to protect the personal data of EU citizens, for consistent and high-quality protection of the natural person, removing obstacles to data transmission within the EU, and addressing exports of personal data to the outside of the union.
%Three major stakeholders are identified in the GDPR\footnote{According to article 4 of the GDPR, for more details see, https://gdpr-info.eu/art-4-gdpr/} that participate in the data processing: 
%\begin{itemize}
%  \item \emph{Data subject}. A natural person whose personal data is being collected, stored and/or processed.
%  \item \emph{Data controller}. An entity (often organization) who is responsible for data processing of a data subject's personal data. A data controller is in control of the processing application. Besides, it has a legal relationship with the data subjects to provide privacy policies and informed data subject consent.
%  \item \emph{Data processor}. A processing entity engaged by the data controller. The data processor is usually a third party external to the company. 
%\end{itemize}
%
%A data protection impact assessment (DPIA)\footnote{Article 35 of the GDPR covers Data Protection Impact Assessments, to read details see, https://gdpr.eu/article-35-impact-assessment/} is a privacy impact assessment aimed at identifying and analyzing how specific data processing activities influence the privacy of data subjects.
%Under the GDPR, a DPIA will be mandatory for any new high risk processing projects, or when profiling activities are carried out using personal data.
%A DPIA can enable organizations to identify, mitigate and prepare for the execution of any risk-related remedies against data protection risks and evaluate the sustainability of a project early. 
% To conduct a DPIA, the GDPR calls for having the following components as described in Article 35: 
% \begin{itemize}
%  \item \emph{a systematic description of the envisaged processing operations and the purposes of the processing, including, where applicable, the legitimate interest pursued by the controller} 
%  \item \emph{an assessment of the necessity and proportionality of the processing operations in relation to the purposes}
%  \item \emph{an assessment of the risks to the rights and freedoms of data subjects}
%  \item \emph{the measures envisaged to address the risks, including safeguards, security measures and mechanisms to ensure the protection of personal data and to demonstrate compliance with this Regulation taking into account the rights and legitimate interests of data subjects and other persons concerned.}
% \end{itemize}
%As we discussed earlier, this assessment differs from the classic risk assessment methodologies since the data controller must perform the assessment in the interest of the data subjects.
%The protection of the rights of data subjects may conflict with the organizations' objectives when companies implement appropriate safety measures while confronting various sorts of restrictions (e.g., budget).
%This paper focuses on a principled methodology to assist data controllers to discover the best deal for each of the stakeholders while maintaining the risk of the data subject within appropriate boundaries.
% the multi-stakeholder risk trade-off analysis problem (MSRToAP) was introduced in our previous work~\cite{mollaeefar2020}.
% To solve MSRToAP cases, we proposed~\cite{mollaeefar2020} a multi-stakeholder risk assessment methodology that gives the risk assessor the ability to estimate the risk-exposed level on a quantitative scale. The proposed methodology, however, does not suggest a risk management policy as an ideal approach for minimizing risk exposure. We make the key addition to this paper by using the multi-objective optimization problem concept to extend and refine our previous methodology. In the following sections, we will explain the methodology in more depth.
%The main problem is to find optimal solutions in presence of (possibly) conflicting multiple objectives.
%Below, we first (Section~\ref{subsec:data-protection}) overview some of the goals related to data protection and then (Section~\ref{subsec:moop}) recall the appropriate notion of optimality.

\subsection{\textbf{Data Protection Goals in Information Security and Privacy}}
\label{subsec:data-protection}
Protection goals play an essential role in analyzing information security in terms of concepts or implementations of data processing systems and guiding the selection of the proper technological or organizational protections for each application~\cite{zwingelberg2011}.
As IT security protection goals, the classical triad of Confidentiality, Integrity, and Availability (also called the CIA triad)---first employed in the early 1980s---would classify the system's security capabilities and controls to achieve a secure outcome~\cite{brooks2017}. 
In recent years, even without any legislative obligations, organizations have taken these three protection goals into account in their own interests. Initially, they developed only for IT security and outline criteria for secure operation, namely the operation of organizational procedures in relation to their business operations. 
Apart from these IT security protection goals, the current data protection legislation (e.g., GDPR) has provided other data protection-specific goals that organizations must also consider when business processes involve processing personal data.
In this regard, in comparison to the IT security goals, the protection goals of data protection require a wider understanding. 

The Standard Data protection Model (SDM)~\cite{fur2017standard} uses the term ‘‘data protection goals’’ to describe certain categories of requirements derived from data protection law.
These requirements are aimed at properties of lawful processing operations, which have to be ensured by technical and organisational measures. 
The SDM specifies the CIA triad, Unlinkability and Data minimization, Transparency, and Intervenability as six protection goals of data protection. The latter three goals aim at the specific protection requirements of data subjects and reflect the data protection requirements in an operational form.
The SDM defines these data protection goals as follows:

\begin{enumerate}[{G}1.]


\item \textit{\textbf{Confidentiality}} refers to the requirement that no person is allowed to access personal data without authorisation.

\item \textit{\textbf{Integrity}} refers, on the one hand, to the requirement that information technology processes and systems continuously comply with the specifications that have been determined for the execution of their intended functions. On the other hand, integrity means that the data to be processed remain intact, complete, and up-to-date.

\item \textit{\textbf{Availability}} is the requirement that personal data must be available and can be used properly in the intended process. Thus, the data must be accessible to authorised parties and the methods intended for their processing must be applied.

\item \textit{\textbf{Unlinkability $\&$ Data minimization}} where the \emph{unlinkability} goal refers to the requirement that data shall be processed and analysed only for the purpose for which they were collected, while the \emph{data minimization} goal covers the fundamental requirement under data protection law to limit the processing of personal data to what is appropriate, substantial and necessary for the purpose. 

\item \textit{\textbf{Transparency}} refers to the requirement that the data subject as well as the system operators and the competent supervisory authorities can identify to a varying extent, which data are collected and processed for a particular purpose, and which systems and processes are used for this purpose, where the data flow to which purpose, and who is legally responsible for the data and systems in the various phases of data processing.

\item \textit{\textbf{Intervenability}} refers to the requirement that the data subjects are effectively granted the right to notification, information, rectification, blocking and erasure at any time.

\end{enumerate}

These protection goals help to structure threats and identify which safeguards need to be implemented~\cite{zwingelberg2011}. In this regard, we will take advantage of these defined protection goals to identify potential threats and their relation with these goals---by mapping each threat to these goals---to evaluate the severity of threats.


%\subsection{\textbf{Multi-Objective Optimization Problem}}
%\label{subsec:moop}
%
%We take a quantitative approach on the fulfillment of the protection goals identified above.  The idea is to be able to introduce appropriate metrics to measure how much a certain objective is not fulfilled so that we can attempt %to minimize this quantity by selecting appropriate security controls.  Indeed, we must do this by considering only those configurations of security controls that are feasible in terms of budget and skills for the various stakeholders involved in the system.  This kind of problem can be formalized as a Multi-objective Optimization Problem (MOOP)~\ref{srinivas1994muiltiobjective}, i.e.  
%\begin{equation}
%    \label{eq:moop}
%    min_{\overline{x}} ~
%     \langle f_1(\overline{x}), ..., f_n(\overline{x}) \rangle 
%     \quad\quad \mbox{subject to} ~\overline{x}\in \mathcal{D}
%\end{equation}
%where $\overline{x}$ is the vector of design variables (in our case, the configuration of the possible security controls to be adopted), $f_i$ is an objective function (intuitively, $f_i$ measures how much an objective is not %fulfilled for the given stakeholder $i$) for $i=1, ..., n$, and $\mathcal{D}$ is the feasible design space, i.e.\ the set of all possible values among which to search for the optimal solutions (in our case the set of configurations %for security controls that are feasible for the various stakeholder in terms of budget or skills).  
%
%In presence of multiple objectives, such as the protection goals identified above, it may be difficult to even define the notion of optimal solution.  In fact, there may be no single solution and it is often necessary to identify a set of solutions fitting a given definition of optimum.  For this, the main concept in defining such a notion of optimum was introduced by Pareto, i.e.\ a point $\overline{x}^{*}\in \mathcal{D}$ is Pareto optimal iff there does not exist another point $\overline{x}\in\mathcal{D}$ such that $f_i(\overline{x}) \leq f_i(\overline{x}^{*})$ for each $i=1, ..., n$ and $f_j(\overline{x}) < f_j(\overline{x}^{*})$ for at least one $j\in \{1, ..., n\}$. In other words, a point is Pareto optimal if there is no other point that improves at least one objective function without detriment to another function.  

%Related to the notion of a Pareto optimality is that of dominance.  
%A vector $\langle f_1(\overline{x}^{*}), ..., f_n(\overline{x}^{*}) \rangle$ of objective functions is non-dominated iff there does not exist another vector $\langle f_1(\overline{x}), ..., f_n(\overline{x}) \rangle$ such that $f_i(\overline{x}) \leq f_i(\overline{x}^{*})$ for each $i=1, ..., n$ with at least one $f_j(\overline{x}) < f_j(\overline{x}^{*})$; otherwise, $\langle f_1(\overline{x}^{*}), ..., f_n(\overline{x}^{*}) \rangle$ is dominated.  
%This means that a Pareto optimal point is often considered the same as a non-dominated point.

%A multi-objective optimization problem (MOOP) deals with more than one objective function, and these objectives are to be minimized or maximized~\cite{srinivas1994muiltiobjective}. 
%In most cases, one solution would not satisfy all objective functions, and the optimal solution of one objective will not certainly be the most desirable solution for other objectives. 
%Therefore, different solutions will produce trade-offs between different objectives, and a set of solutions is required to represent the optimal solutions of all objectives. 
% A variety of algorithms have been proposed to solve a multi-objective problem by researchers. 
%To fully perceive MOOP and the algorithms that solve these kinds of problems, some concepts and definitions must be clarified. In following some most important of these concepts are mentioned:
%\begin{itemize}
%\item \textbf{Decision variables and objective space}

%The variable bounds of an optimization problem restrict each decision variable to a lower and upper limit which defines a space called decision variable space. In multi-objective optimization values of objective functions create a multi-dimensional space called objective space. Each decision variable on variable space corresponds to a point in objective space.
%\end{itemize}


%\begin{itemize}
%\item \textbf{Dominance relation}

%Optimizing a solution with respect to one objective will not result in an optimal solution regarding the other objectives. For instance, solution $X_1$ dominate solution $X_2$ :
%(i) if $X_1$ is no worse than $X_2$ with respect to all objectives value, and (ii) solution $X_1$ is strictly better than solution $X_2$ in at least one objective value. Therefore, solution $X_1$ dominates solution $X_2$, solution $X_1$ is non-dominated by solution $X_2$, or solution $X_2$ is dominated by solution $X_1$.
%\end{itemize}


%\begin{itemize}
%\item \textbf{Pareto-optimal set (non-dominated set)}

%A solution is Pareto-optimal if it is not dominated by any other solution in the variable space. The Pareto-optimal is the best known (optimal) solution with respect to all objectives and cannot be improved in any objective without worsening in another objective. The set of all feasible solutions that are non-dominated by any other solution is called the Pareto-optimal or non-dominated set~\cite{marler2004survey}. 
% If the non-dominated set is within the entire feasible search space, it is called globally Pareto-optimal set. 
%It is important to note that the feasible objective space contains not only Pareto-optimal solutions but also solutions that are not optimal. In fact, feasible objective space can divide into two set solutions, a Pareto-optimal and a non-Pareto-optimal set~\cite{srinivas1994muiltiobjective}.
%\end{itemize}


% \subsection{\textbf{Threat Modeling Methodologies}}



 

%
% The objectives of availability, integrity and confidentiality thus also serve to guarantee information security in public authorities and companies, i. e. to secure and protect the data of an organisation.
% It presents the perspective of the data subject whose rights are at stake. 
% The protection goals Integrity, Availability, Confidentiality, Transparency, and Data Minimisation can be found conceptually in the regulation text while also referring to IT security requirements. Unlinkability and Intervenability have been adopted as data protection goals in numerous individual articles of the GDPR, among other things, via the principle of purpose limitation, erasure, and data portability.

==> Removed/Discussion.tex <==
\section{Discussion}\label{sec:discuss}

The multi-stakeholder risk assessment methodology described above has two primary purposes. 
First of all, characterizing an approach to ascertain each stakeholder's risk exposure levels when the threats have been identified in a given system, and second, proposing an efficient method to solve the Multi-Objective Risk Minimization Problem which makes to discover appropriate solutions or, in another, word Pareto-optimal solutions. 
% To achieve these purposes, we have proposed a multi-stakeholder cybersecurity risk assessment methodology which consists of two main phases,
The process flow of the methodology is illustrated in Figure~\ref{fig:methodology}, where the first phase of the proposed methodology meets our first purpose while the second phase is devoted to achieving the second purpose. 
The proposed methodology enables software designers and security and privacy experts to overview potential risks in the system and analyze the requirements from multiple viewpoints. This allows them to perform a trade-off between RMPs to select appropriate risk management policy, which comprises both technical and organizational measures to minimize risks.

As a preliminary step, the risk analyst needs to provide three input artifacts for the purpose of performing the risk impact analysis. This step is critical from a security and privacy standpoint because it assists software designers in understanding security and privacy threats and how those threats impact stakeholders, particularly data subjects, and it assists the organization as the data controller in identifying possible security and privacy countermeasures to mitigate the risk of potential threats. 

The first phase is partially automated, and it needs the risk analyst intervention to prepare the required documents for the automated phase. In the first phase, apart from determining stakeholders and their protection criteria process for the given system that the risk analyst must determine, he/she is asked to (i) assign an impact level for each threat for all determined stakeholders' preferences which is called \textit{Threat-Preference Association}, (ii) map the identified threats to data protection goals which called \textit{Threat-Protection Goals Association}, and (iii) provide a list contains threats and their related controls, as well as define the implementation finite set values (e.g., we considered three possible values \{0,0.5.1\}) to calculate $TE$ values and finally the feasible set be generated. The output of this process will be a list of distinct $TE$ values.
% Therefore, it is important to note that making an effort to find all of the potential threats, as well as their controls, can aid in the development of a more accurate risk impact assessment.

% The first phase is called \emph{Threat Modeling}, which supports software designers in understanding security and privacy threats and how those threats impact stakeholders, particularly data subjects, and helps the organization as the data controller identify possible security and privacy countermeasures to alleviate potential attacks. 
% This phase produces comprehensive system documentation through security and privacy-aware specification of the data processing activities to identify potential adverse events, in other words, identifying threat scenarios. The last step in this phase is dedicated to finding possible security and privacy countermeasures that may relieve the risk of identified threats.

% The risk impacts evaluate in the first phase for all involved stakeholders through some defined processes. The first process that needs to be taken into account in this phase is determining stakeholders’ impact criteria and weights, and then we can specify the association between the identified threat in the previous phase and these criteria. Through this, the \emph{impact levels} will evaluate. 
% \emph{Threat criticality quantification} is another process that demands to be performed in this phase, which estimates how dangerous and critical these threats among themselves. In other words, this process aims to prioritize the threats in terms of harmfulness. To do this prioritization, we take advantage of the \emph{Data Protection Goals} and \emph{Threat Existence} concepts. The former concept is aimed to specify the association between these goals and the identified threats, whereas the latter says about how likely threats exist in the given system through estimating controls’ implementation status levels for each threat. Finally, in this phase, the risk assessment becomes fulfilled by multiplying the two obtained values from the described process above (impact levels and threat criticalities), and then the risk impact calculates for all involved stakeholders. 

\begin{figure} [!t]
    \centering
	\includegraphics[width=0.95\textwidth]{Figures/AllSolutionPoints.JPG}
    \caption{All feasible solutions in our scenario.}
    \label{fig:AllPoints}
\end{figure}

The second phase is a fully automated procedure where the results obtained from the first phase will process under some defined processes. Indeed, in this phase, the risk exposure levels will calculate to apply an optimization algorithm to find the optimal solutions. By having the assigned impact levels as input that are obtained from the previous phase, the risk impacts for each stakeholder will evaluate under the \emph{impact level evaluation} process.
\emph{Threat Criticality Quantification} is another process that demands to be performed in this phase, which estimates how dangerous and critical these threats are among themselves. In other words, this process aims to prioritize the threats in terms of harmfulness. 
By multiplying the two obtained values from the described processes above,
the risk assessment becomes fulfilled. Then as the final process in this phase, we require to solve a multi-objective optimization problem that is optimization problem that involves multiple objective functions, which in our case are the risk exposure levels from multiple points of view. The optimal solutions are obtained by applying the Pareto-Optimality algorithm. 
\begin{table}[!b] \centering
\caption{Pareto solutions with the defined risk exposure boundary.}
\label{tab:Pareto-solutions}

\begin{tabular}{c|c|c}
% \toprule
Pareto Solutions & Data Subject & Data Controller \\ \hline\hline
$\mathbb{S}_1$ & 0.4514       & 0.5518          \\ 
$\mathbb{S}_2$ & 0.4503       & 0.5536          \\
$\mathbb{S}_3$ & 0.4504       & 0.5530          \\
$\mathbb{S}_4$ & 0.4520       & 0.5501          \\
$\mathbb{S}_5$ & 0.4516       & 0.5502          \\
$\mathbb{S}_6$ & 0.4505       & 0.5525          \\ 
% \bottomrule
\end{tabular}
\end{table}
% In a nutshell, the two phases mentioned above aim to characterize the system to identify potential threats and specify suitable countermeasures to mitigate risk exposure levels for all involved stakeholders, particularly data subjects.
% In the last phase of the proposed methodology, we assist designers and especially data controllers by representing the optimal solutions where the risks are minimized for all participants. To do this support, we require to solve a multi-objective optimization problem that is an optimization problem that involves multiple objective functions. In our case, the objective functions are minimized risk exposure levels for all involved stakeholders. To solve this problem, we have proposed an efficient method to generate all possible solutions for a given system. The method significantly reduced the size of the feasible set, which makes we be able to apply the optimization algorithm to find Pareto optimal solutions. All the required steps to solve the multi-objective problem have been explained in detail in Section~\ref{sec:optimization}.

\begin{table}[!b] \centering
\caption{Retrieved $x_T$ values for the identified solution.}
\label{tab:Retrieve-solutions}
\begin{tabular}{c|ccccc} 
% \toprule
    & $x_{T_1}$ & $x_{T_2}$& $x_{T_3}$& $x_{T_4}$ & $x_{T_5}$ \\\hline\hline
$\mathbb{RS}_1$     &$0.9$&$0.4$&$0.75$&$1$&$0.25$\\
$\mathbb{RS}_2$     &$0.8$&$0.4$&$0.875$&$0.66$&$0.33$ \\
$\mathbb{RS}_3$     &$0.6$&$0.3$&$0.875$&$0.33$&$0.33$\\
$\mathbb{RS}_4$     &$0.6$&$0.25$&$0.75$&$0.25$&$0.25$ \\
$\mathbb{RS}_5$     &$0.6$&$0.2$&$0.25$&$1$&$0.25$\\
$\mathbb{RS}_6$     &$0.5$&$0.25$&$0.875$&$0.16$&$0.33$ 
% \bottomrule
\end{tabular}
\end{table}


We have plotted all possible solutions as the feasible set in our scenario in Figure~\ref{fig:AllPoints}, and each point in this plot expresses a solution under an RMP. In this figure, the data subject’s risk exposure level is plotted on the x-axis, where the y-axis shows the risk exposure level for the data controller. In this figure, the optimal solution is the point in the left side bottom where the risk exposure levels for the data subject and the data controller equals 0.2260 and 0.4168, respectively. 
This solution point dominates all other solutions in this figure. However, this point may not be the best choice that the risk analyst may look. In this regard, we can define a boundary of risk exposure levels and then apply the optimization algorithm to find Pareto points. For example, if we set the minimum risk exposure level for the data subject and the data controller 0.45 and 0.55, respectively, the obtained Pareto points in our scenario are the same as reported in Table~\ref{tab:Pareto-solutions}. 


% One point that needs to be said is that, once the risk analyst selects a solution as an optimal solution, he can understand under which RMP this solution has obtained, and consequently, he learns the value of each TE, which means he is able to configure controls in different combination in terms of implementation statuses to reach the acquired TE values. 
One point that should be mentioned here is that, once a solution has been identified as an optimal solution, the risk analyst can realize under which RMP this solution has been identified, and as a result, he learns the value of each $x_T$. This means that the risk analyst is able to configure controls in different combinations in terms of implementation statuses in order to achieve the acquired $x_T$ values. 
For example, in Table~\ref{tab:Retrieve-solutions}, we have retrieved possible $x_T$ values for the identified solutions in the previous table.


%  Possible implementation combinations based on the example above 
% [0.5, 6.0, 1.0, 0.0, 1.5]
% -------------
% [1.0, 6.0, 0.5, 1.0, 2.0]
% -------------
% [2.0, 7.0, 0.5, 2.0, 2.0]
% -------------
% [2.0, 7.5, 1.0, 1.5, 1.5]
% -------------
% [2.0, 8.0, 3.0, 0.0, 1.5]
% -------------
% [2.5, 7.5, 0.5, 2.5, 2.0]


\subsection{\textbf{Implementation}}
We have implemented the proposed risk assessment methodology in the Java. The tool has two main objectives, (i) to evaluate and quantify risk levels for all involved stakeholders and (ii) to solve the risk minimization problem, which is a multi-objective optimization problem. The tool works with JSON files, all inputs and outputs, and the repository of the tool is available on GitHub\footnote{https://github.com/Majid-Mollaeefar/MSRMP}.



\subsection{\textbf{Experimental result}}

% Before performing the experimental analysis, we need to know the analysis’s objective and what parameters must be considered. This analysis aims to see how the size of the solution set changes under different scenarios and how much this size reduces with the proposed method, and the computation time required for this set to be created. 
To perform the experimental analysis, first of all, we need to determine the objective of the analysis as well as the parameters that must be taken into consideration.
The objective of this analysis is to determine how the size of the solution set changes under different circumstances, how much the size of the solution set decreases with the proposed method, and how much computing time is required to generate the solution set.
As we learned in the previous section, the solution set size contains all possible solutions created by multiplying TE variables, depending on two variables, (i) the number of threats and (ii) the number of controls. 

In table~\ref{tab:experimental}, we have reported some experimental results of the proposed method with the aim of computing the required solution set size according to the number of threats and controls that have been involved for a given system. We have arranged this analysis for two different sizes of controls per each threat, where the first column reports these two sizes that are assigned to each threat.
This analysis is done on the different range of threats (five to eight threats) reported on the second column, and consequently, the total number of controls for each of these scenarios has been reported in column three. 
In order to generate all possible solutions for each scenario, the required solution set size is computed in both non-optimized and optimized (our method to obtain all possible solutions) methods in column fourth. For example, in the first row, the solution set size for the non-optimized method equals $3^{20}$, where through the proposed method, the size of the solution set is only $32768$, which to compare the former method has around one hundred thousand times reduction. As can be seen, this reduction grows for the large-size scenarios in terms of the number of threats and controls. This comparison is shown in column fifth, and the required computation times are reported in column six. In the last column, we have also measured the maximum size of RAM heap space that has been used in our proposed method to generate the solution sets.
% \begin{table}[!b]\center
% 		\caption{Experimental result.}
% \includegraphics[width=0.98\textwidth]{Figures/Experimental.pdf}
% \label{tab:experimental}
% \end{table}

% point out why the method is more efficient in terms of generating all possible solutions 
% \begin{table}[] 
\begin{sidewaystable}
\centering
\caption{Experimental results}
% \begin{adjustbox}{angle=90}
\label{tab:experimental}
% \scriptsize
\begin{tabular}{ccccccc}
\toprule
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Threat \\($\mathcal{T}$)\end{tabular}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Number of Controls\\ per Threat\end{tabular}} &
  \multicolumn{2}{c}{Solution Set Size} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Reduction \\ Factor (Million)\end{tabular}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Computation \\ Time (MS)\end{tabular}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Maximum RAM \\ Heap Size (MB)\end{tabular}} \\ 
  \cmidrule(lr){3-4}      &    & $k^{|C|}$ & $\Pi_{T\in \mathcal{T}} |{X}_T|$   &            &         &            \\ \midrule
5 & \multirow{4}{*}{4} & $3^{5*4}$           & $32,768$      & $\sim$0.1  & 312     & $\sim$0.25 \\
                  6 &  & $3^{6*4}$          & 262,144     & $\sim$1    & 1,212    & $\sim$1.5  \\
                  7 &  & $3^{7*4}$          & 2,097,152   & $\sim$11   & 9,774    & $\sim$12   \\ 
                  8 & & $3^{8*4}$          & 16,777,216  & $\sim$110  & 237,124  & $\sim$29   \\ \midrule
                  5 &\multirow{4}{*}{5} & $3^{5*5}$           & 100,000     & $\sim$8    & 626     & $\sim$0.5  \\
                  6 &  & $3^{6*5}$          & 1,000,000   & $\sim$205  & 3,753    & $\sim$9    \\
                  7 &  & $3^{7*5}$           & 10,000,000  & $\sim$5K   & 105,292  & $\sim$28   \\
                  8 &  & $3^{8*5}$           & 100,000,000 & $\sim$121K & 2,787,441 & $\sim$416  \\ \bottomrule

% \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Number of Controls\\ per Threat\end{tabular}} &
%   \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Threat \\Set Size\end{tabular}} &
%   \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Total\\Controls\end{tabular}} &
%   \multicolumn{2}{c}{Solution Set Size} &
%   \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Reduction \\ Factor (Million)\end{tabular}} &
%   \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Computation \\ Time (MS)\end{tabular}} &
%   \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Maximum RAM \\ Heap Size (MB)\end{tabular}} \\ 
%   \cmidrule(lr){4-5}   &   &    & Full & Reduced   &            &         &            \\ \midrule
% \multirow{4}{*}{4} & 5 & 20 & $3^{20}$           & $32,768$      & $\sim$0.1  & 312     & $\sim$0.25 \\
%                   & 6 & 24 & $3^{24}$          & 262,144     & $\sim$1    & 1212    & $\sim$1.5  \\
%                   & 7 & 28 & $3^{28}$          & 2,097,152   & $\sim$11   & 9774    & $\sim$12   \\ 
%                   & 8 & 32 & $3^{32}$          & 16,777,216  & $\sim$110  & 237124  & $\sim$29   \\ \midrule
% \multirow{4}{*}{5} & 5 & 25 & $3^{25}$           & 100,000     & $\sim$8    & 626     & $\sim$0.5  \\
%                   & 6 & 30 & $3^{30}$          & 1,000,000   & $\sim$205  & 3753    & $\sim$9    \\
%                   & 7 & 35 & $3^{35}$           & 10,000,000  & $\sim$5K   & 105292  & $\sim$28   \\
%                   & 8 & 40 & $3^{40}$           & 100,000,000 & $\sim$121K & 2787441 & $\sim$416  \\ \bottomrule
                   
\end{tabular}
\end{sidewaystable}


%  \input{Sections/Algorithms}

==> Removed/Impact_Assessment.tex <==
\section{Mappings and Associations}\label{sec:impact-assessment}
% The second phase is the heart of the impact assessment.
\begin{table}[!b] \center
    \caption{An example of possible threat scenarios and their possible malicious activity in the ACME scenario}
    \includegraphics[width=0.99\textwidth]{Figures/Threat-table.pdf}
    \label{tab:threat-table}
\end{table}
\begin{table}
\caption{The assigned impacts to each stakeholders' preferences for each threat in our scenario}
\label{tab:threat-preference-association}
\resizebox{\textwidth}{!}{\begin{tabular}{c|l|c|ccccc}

\multirow{2}{*}{Stakeholder} &
  \multicolumn{1}{c|}{\multirow{2}{*}{Preferences}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Weights\\ (PW)\end{tabular}} &
  \multicolumn{5}{c}{Impact Values (IV)} \\ \cline{4-8} 
                                 & \multicolumn{1}{c|}{}  &     & T1 & T2 & T3 & T4 & T5 \\ \hline \hline
\multirow{4}{*}{Data Subject}    & Health   condition     & 0.4 & 0  & 4  & 0  & 3  & 4  \\ 
                                 & Individual freedom     & 0.2 & 0  & 2  & 4  & 3  & 3  \\ 
                                 & Social situation       & 0.3 & 1  & 2  & 3  & 0  & 3  \\ 
                                 & Financial   situation  & 0.1 & 0  & 3  & 1  & 0  & 3  \\ \hline
\multirow{2}{*}{Data Controller} & Reputational situation & 0.4 & 1  & 2  & 3  & 2  & 2  \\  
                                 & Financial   situation  & 0.6 & 2  & 2  & 3  & 3  & 2  \\ 
\end{tabular}}
\end{table}

\begin{table} \center
\caption{Affected protection goals by each threat and the observation weights in our scenario, G1= Confidentiality, G2= Integrity, G3= Availability, G4= Unlinkability $\&$ Data minimization, G5= Transparency, and G6= Intervenability. }
\footnotesize
\label{tab:Threat-Goals}

\resizebox{\textwidth}{!}{\begin{tabular}{c|cccccc|c}
% \hline
\multicolumn{1}{c|}{\multirow{2}{*}{Threat}} &
  \multicolumn{6}{c|}{Data Protection Goals} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Observation\\ Weights (OW)\end{tabular}} \\ \cline{2-7}
\multicolumn{1}{c|}{} & G1 & G2 & G3 & G4 & G5 & G6 &      \\ \hline \hline
T1                     & \ding{53}  & -  & -  & \ding{53}  & -  & -  & 2/10 \\ 
T2                     & \ding{53}  & \ding{53}  & \ding{53}  & -  & -  & -  & 3/10 \\ 
T3                     & \ding{53}  & -  & -  & \ding{53}  & -  & -  & 2/10 \\ 
T4                     & -  & \ding{53}  & \ding{53}  & -  & -  & -  & 2/10 \\ 
T5                     & -  & -  & -  & -  & -  & \ding{53}  & 1/10 \\ 
\end{tabular}}
\end{table}

In risk management, the impact assessment is a critical task because it aims to estimate the potential consequences of threats and how stakeholders evaluate them. 
It is mostly a subjective evaluation, which makes it particularly critical when attempting to estimate the impact from third parties' point of view, such as the data subject.
We accept this subjectivity level as unavoidable, but we mitigate it by conceiving a cross-weighting system, making impact assessment more systematic. 
In a nutshell, in such a weighting system, the risk analyst must provide his/her opinion about the potential impact of threats.
However, he/she is asked for an opinion multiple times and on different aspects of the problem (i.e., by considering stakeholder's preferences), with the twofold objective of (i) inducing the risk analyst to consider multiple points of view and (ii) merging these points of view into a more balanced value. In this phase, the following processes need to be done:

\subsection{\textbf{Determining Stakeholders' Preferences}}~Different stakeholders have different criteria that define what they consider risky. Data controllers (e.g., companies) typically choose business impact criteria, such as financial impact or reputation, whereas data subjects (e.g., individuals) evaluate risk based on impact on their personal sphere. In our scenario, we have considered the \textit{social situation, individual freedom, financial situation}~\cite{ref_article4}, and \textit{health condition} as the data subject impact criteria. \textit{Reputational situation} and \textit{financial situation} are the impact criteria for ACME, which are linked to indirect and direct pecuniary loss or damage. Additionally, each stakeholder has different preferences, which result in different importance given to different criteria. For instance, in our scenario, the health condition criterion is more momentous than the others for patients. We capture these high-level stakeholder preferences by assigning a weight to each stakeholder’s preference. 
The associations between stakeholders and preferences with weights are shown in the first three columns of Table~\ref{tab:threat-preference-association}.
This step’s output will be the list of stakeholders and their preferences and an assigned weight to each of them, which is the input for the next process.

\subsection{\textbf{Threat-Preference Association}}
% \begin{table}[!b] \center
%     \caption{The assigned impacts to each stakeholders' preferences for each threat in our scenario}
%     \includegraphics[width=0.99\textwidth]{Figures/Threat-preference-association.pdf}
%     \label{tab:threat-preference-association}
% \end{table}


Each threat is perceived as more or less dangerous by each stakeholder in relation to his/her own criteria. For example, it is very unlikely that excessive storage of patients’ health data would damage ACME’s reputation. On the other hand, by increasing stored data on its data storage, there is financial damage on ACME cause of cost of storage and management of the IT infrastructure. The reputation of patients is not affected by excessive storage of personal data. However, the increasing amount of stored data increases the risk and impact of data breaches and leaks. 
To capture this association, we assign a value to the level of aversion that each stakeholder is considered to have against each threat, according to his/her own criteria. This value intends to capture the contribution of that specific preference to the overall evaluation of the risk impact. In Table~\ref{tab:threat-preference-association}, we have assigned an impact value in a scale from 0 to 4 (0-no impact, 1-low, 2-moderate, 3-critical, 4-catastrophic) to each stakeholder’s preference for each identified threat in our scenario. 


% \subsection{\textbf{Selecting data process principles}}
\subsection{\textbf{Threat-Protection Goals Association}} \label{sec:threat-principle}

As we observed earlier in Section~\ref{sec:Back}, six protection goals have been specified by the SDM~\cite{fur2017standard}. 
These protection goals reflect the protection objectives in information security and present the data subject’s perspective, whose rights are at stake.  
Generally, each threat has potentially an impact on one or more protection goals, which depends on the threat’s nature. For example, every “\emph{Denial of service}” threat will intuitively have more impact on data availability rather than on integrity, while any “\emph{Identity theft}” will have more impact on data confidentiality. 
\emph{Threat-Protection Goals association} is the action of mapping the data protection goals to the list of threats as derived by the threat scenario identification process in Figure~\ref{fig:methodology}. For example, we have mapped these protection goals to the identified threats. This association is shown in Table~\ref{tab:Threat-Goals}, where the “\ding{53}” mark in a cell means the associated goal (in column) is affected by the threat (in row).
The more a threat impacts multiple goals, the more it is considered pervasive (e.g., threat $T2$ is the most pervasive in Table~\ref{tab:Threat-Goals} as it affects 3 goals); the more a goal is impacted by multiple threats, the more it is considered scattered (e.g., goal $G1$ is the most scattered in Table~\ref{tab:Threat-Goals} as it impacts 3 threats). Notice that  this association does not directly affect the threat impact because a goal impacted severely by a single threat can be more threatened than a goal impacted slightly by many threats. This information is used in combination with others to derive the impact. We introduce the “\textit{Observation Weight}” for each threat according to the number of protection goals affected by the threat with respect to all affected protection goals in total. For simplicity, we assume all the protection goals have equal importance. For example, in Table~\ref{tab:Threat-Goals}, the observation weights are computed through Formula~\ref{eq:OW} for each threat in our scenario.
\begin{equation} \label{eq:OW}  
    \forall_{T=1,..,t} ~~ OW_{{T(i)}}= \frac{NG_{T(i)}}{{\sum_{i=1}^{t}NG_{T(i)}}}
\end{equation}
where $NG_{T(i)}$ represents the number of affected goals by ith threat. For example, according to Table~\ref{tab:Threat-Goals}, $OW_{T1}$ is $2/10$, where $G1$ and $G4$ are two affected goals by $T1$ and sum all affected goals equals 10.  
% This process is the same as the previous approach, only with this difference; instead of quantifying the criticality of threats based on impacted protection goals, we quantify them based on data processing principles. 
% \begin{table}[!b] \center
%     \caption{Affected protection goals by each threat and the observation weights in our scenario}
%     \includegraphics[width=0.95\textwidth]{Figures/Threat-Goals.pdf}
%     \label{tab:Threat-Goals}
% \end{table}



\subsection{\textbf{Threat Existence Calculation}}
\label{sec:threat-existence}
We define threat existence ($TE$) value as the impact residue of a threat after the adoption of a set of controls to reduce the risk of its occurrence. To better understand how the \textit{threat existence value} calculates, in Table~\ref{tab:threat-control}, we have associated a set of controls to each identified threat in our scenario.
In this table, an implementation status is also assigned to each control, and each threat has a truth value from 0 to 1, which is computed by using the implementation statuses. 
The value $TE$ is calculated through Formula~\ref{eq:threat-existence}. In this formula, $a_{T(i)}(j)$ represents the implementation status of the $jth$ control for threat $i$. 
\begin{align} 
TE_{(i)} = 1- \frac{\sum_{j=1}^{J}a_{T(i)}(j)}{J}
\label{eq:threat-existence} 
\end{align}
Through back to the problem formalization (Section~\ref{subsec:problem}) where we defined $m_T(C)$ and if we compare it with the formula above, we realize $m_T(C)$ = $\frac{\sum_{j=1}^{J}a_{T(i)}(j)}{J}$. Note that, as we mentioned earlier, each of these controls can have an implementation status value in the range of the finite set \{0, 0.5, 1\}, which represents the control not implemented, partially and fully implemented, respectively.
By looking again to the process flow in Figure~\ref{fig:methodology}, the output of this phase is to list all distinct $TE$ values. To this end, we need to perform an extra process which generates the suitable feasible set that will use as an input for the \textit{Threat Criticality Quantification} process in the next phase.

\begin{table}[!b]\center
		\caption{The associated controls to each threat and the implementation statuses together with computed threat existence values.}
\includegraphics[width=0.98\textwidth]{Figures/Threat-controls.pdf}
\label{tab:threat-control}
\end{table}


\subsection{\textbf{Feasible Set Generation}}
This process is critical because it makes the investigation for finding Pareto-optimal solutions (i.e., the final result of the methodology) be applicable. Thus, as last step of this phase and before finding Pareto-optimal solutions for our scenario, we must determine the feasible solutions set.
Through back to Examples 4 and 5 in the problem formalization (Section~\ref{subsec:problem}), we can understand the number of variables (for our multi-objective problem) are the sum of controls $N=C_{T1}+C_{T2}+...+C_{Tt}$. For example, as you can see in Table~\ref{tab:threat-control}, the total number of controls equals $N=C_{T1}+C_{T2}+C_{T3}+C_{T4}+C_{T5}=25$. 
% Before finding Pareto-optimal solutions for an MSRMP, we must determine the feasible solutions set.
% As we pointed out earlier, in an MSRMP for each identified threat, there is a set of controls associated with threats. So we can summarize the optimization problem as follows: 
% \begin{itemize} 
% \item{A set of threats \{$T_1, T_2,..., T_t$\}.}
% \item{A set of mitigation controls that are divided into a list of subsets \{$C_{T1}, C_{T2}$
% $,..., C_{Tt}$\} where each subset contains a list of controls that are determined for each threat. Each of these controls can have an implementation status value in the range of the finite set \{0, 0.5, 1\}, which represents the control not implemented, partially and fully implemented, respectively.}  
% \end{itemize}
% From these considerations, we can understand the number of variables (for our multi-objective problem) are the sum of controls $N=C_{T1}+C_{T2}+...+C_{Tt}$. For example, as you can see in Table~\ref{tab:threat-control}, the total number of controls equals $N=C_{T1}+C_{T2}+C_{T3}+C_{T4}+C_{T5}=25$.
Therefore, the feasible set is the set of all possible values that can be assigned to the variables. In the case of $N$ variables, the feasible set will have $3^N$ feasible solutions corresponding to all possible assignments of one among three possible values \{0, 0.5, 1\} to each of the $N$ variables.
However, generating the feasible set in this way is almost impractical due to the exponentially growing number of possible solutions. 
For instance, for Table~\ref{tab:threat-control} with 25 controls, the feasible set space would be more than 847 billion solutions, and it is not possible to investigate this significant space to find Pareto-optimal solutions. 
The way of considering all possible permutation of control values to build the feasible set causes the search space to be increased remarkably. 
Despite the produced solutions being unique in terms of implementation status values for each control, the computed $TE$ values and further in the next phase objective functions (i.e., the risk exposure results in our case) with the identical value will be enormous. 
% In the following, we propose a method to eradicate the repetitive computed objective functions. 

\begin{table}[!b]\center
    \centering
    \caption{All distinct TE values for T1}
    \small
    \begin{tabular}{c|c|c}
    %  {p{2cm}m{0.30\textwidth}m{0.30\textwidth}} 
        % \toprule
         Threat & \multicolumn{1}{c|}{Controls' status summation} & Threat Existence (TE)
         \\ 
         \hline\hline
         \multirow{10}{*}{\begin{tabular}[c]{@{}l@{}}T1-Unlimited \\data storage\end{tabular}}
        %  \multirow{10}{*}{\begin{tabular}[ht]{p{1.98cm}}T1-Unlimited \\data storage\end{tabular}}
        %  $T1$-Unlimited data storage} 
                     & 0.0 & $TE_{1}$ = $1- (0.0)/5$ = 1.0   \\
                     & 0.5 & $TE_{1}$ = $1- (0.5)/5$ = 0.9  \\
                     & 1.0 & $TE_{1}$ = $1- (1.0)/5$ = 0.8  \\
                     & 1.5 & $TE_{1}$ = $1- (1.5)/5$ = 0.7  \\
                     & 2.0 & $TE_{1}$ = $1- (2.0)/5$ = 0.6  \\
                     & 2.5 & $TE_{1}$ = $1- (2.5)/5$ = 0.5   \\
                     & 3.0 & $TE_{1}$ = $1- (3.0)/5$ = 0.4   \\
                     & 3.5 & $TE_{1}$ = $1- (3.5)/5$ = 0.3   \\
                     & 4.0 & $TE_{1}$ = $1- (4.0)/5$ = 0.2   \\
                     & 4.5 & $TE_{1}$ = $1- (4.5)/5$ = 0.1 \\ 
                    %  \bottomrule
                     
    \end{tabular}
    
    \label{tab:example}
\end{table}

% \subsubsection{\textbf{Discover all Pareto-Optimal Solutions for an MSRMP}}
As we described earlier, the $TE$ value (Formula~\ref{eq:threat-existence}) for each threat is the key value (regardless of what the impact level of threat is, which depends on the stakeholder's criteria) for estimating the risk exposures or, in other words, computing the objective functions. Indeed, the $TE$ value represents how much a threat can be dangerous with respect to the implementation status of its associated controls. For example, in the light of Table~\ref{tab:threat-control}, for the first threat ($T1$), $TE_1$ through using Formula~\ref{eq:threat-existence} would be $TE_1 = 1- (1+1+0.5+0.5+0)/5 = 0.4$. What would be $TE_1$ by exchanging the implementation status of $C_{T1}(2)$ with $C_{T1}(5)$ which means the control \textit{“Enabling data deletion”} is fully implemented and the control \textit{“Ensuring limited data processing”} is not implemented? It results in the same value ($TE_1 = 1- (1+0+0.5+0.5+1)/5 = 0.4$).

From this consideration, by establishing a method to find all distinct $TE$ values that a threat can obtain, the feasible set would be built with the incredibly decreased solutions space. Thus, the problem of growing solution space can be reduced to finding all distinct values for the sum $C_{T(i)}$ that range over the finite set \{0, 0.5, 1\} where $i$ represents the $ith$ threat, consequently generating all distinct $TE$ values for each threat.
For instance, in Table~\ref{tab:example}, we have listed all distinct $TE$ values that $T1$ might have, where they are computed by the sum of the implementation status of its controls.
% we have listed all distinct $TE$ values for the sum of implementation status controls for $T1$ along with the computed threat existence values. 
Through Formula~\ref{eq:distinct}, we able to compute the total number of distinct $TE$ values for each threat, where $NC_{T(i)}$ is the number of associated controls to threat $i$, e.g., according to Table~\ref{tab:example}, the  total number of distinct $TE$ values for $T1$ equals $10$. 
Then, by multiplying these values (Formula~\ref{eq:solutions}), the size of the feasible set determines for an MSRMP. In other words, this formula computes the permutation of the determined distinct $TE$ values.
\begin{equation}
    \forall_{i=1,..,t} ~d(i)= (NC_{T(i)} \times 2)
\label{eq:distinct} 
\end{equation} 
\begin{equation}  
\forall_{i=1,..,t}~Feasible~ Set~ Size = d(i) \times d(i+1) \times ...\times d(t) 
\label{eq:solutions} 
\end{equation}

Therefore, in this way, the size of the feasible solutions set is reduced by eradicating repetitive $TE$ values for each threat. To better perceived this reduction, the needed space for our example in Table~\ref{tab:threat-control} would be $d(1)\times d(2)\times d(3)\times d(4)\times d(5) = 10\times20\times8\times6\times6 = 57600$, which more than eight million times smaller to compare with the former method ($3^N$).

% \begin{table}[!b]\center
% 		\caption{All distinct $TE$ values for T1 }
% \includegraphics[width=0.95\textwidth]{Figures/TE-Distinct-Value.pdf}
% \label{tab:example}
% \end{table}
% 


% \textcolor{red}{add some examples of associations}
% In this process, we map each threat to one (or more) data processing principle(s) that demonstrate the lack of compliance with which principle(s) may result in the threat happening. On the other hand, we could realize which principles are more important in connection with the identified threat scenarios through this process. The more threats arise due to incompliance with a principle, the more it is considered a weak point to comply with GDPR. Also, the more a threat impacts on multiple principles, the more it is considered dangerous. 
% Notice that the \textit{threat-principle association} does not directly inform on the threat impact because a principle impacted severely by a single threat can be more threatened than a principle impacted slightly by many threats. However, it is information that is used in combination with others to derive each threat’s impact. 
% For example, in our scenario, we have mapped each identified threat scenario to a (or more) principle(s), and we have shown this relation earlier in Table~\ref{tab:threat-table}.
% Data processing principles set out obligations for organizations (data controllers and processors) that collect, process, and store data subjects' personal data. Six principles have been identified for data processing activities to be GDPR compliant. Companies considering all principles will guarantee that they comply with the data protection regulations. These principles are as follows: 
% \begin{enumerate}[{P}1.]
    

% \item \textbf{Lawfulness, Fairness and Transparency.}~Personal data should be processed lawfully, fairly and in a transparent manner.

% \item \textbf{Purpose Limitation.}~Personal data should be processed for "specified, explicit and legitimate purposes". In other words, the purpose of processing shall be specified before the processing starts and respected throughout the whole personal data life-cycle. 

% \item \textbf{Data Minimisation.}~Personal data shall be "adequate, relevant and limited to what is necessary in relation to the purposes for which they are processed". 

% \item \textbf{Accuracy.}~Personal data shall also be "accurate and, where necessary, kept up to date". This principle is closely related to data subjects’ rights of access and rectification, in other words, data subjects allowed to exercise certain rights in relation to their personal data.

% \item \textbf{Storage Limitation.}~Personal data shall be "kept in a form which permits identification of data subjects for no longer than is necessary for the purposes for which the personal data are processed". 

% \item \textbf{Integrity and Confidentiality (Security).}~Personal data should also be "processed in a manner that ensures appropriate security of the personal data, including protection against unauthorised or unlawful processing and against accidental loss, destruction or damage, using appropriate technical or organisational measures".
% In fact, it concerns the broad concept of information security, which means that suitable security measures need to be taken to prevent personal data not being compromised, whether accidentally or deliberately.
% \item \textbf{Accountability.}~The accountability principle is a new and important addition in the GDPR. According to \textit{Article 5(2)} of the GDPR, the controller shall be responsible and able to demonstrate compliance with all the principles of the GDPR.
% \end{enumerate}

% This process is substituted with \emph{Threat-Goal Correlation} process of our previous approach. The reason behind this changing is that, in the threat modeling phase, we have already correlated security and privacy properties (which can be considered as protection goals) to each threat.

% For example, every “Denial of service” threat will intuitively have more impact on data availability rather than on integrity, while any “Identity theft” will have more impact on data confidentiality.


% The Standard Data protection Model (SDM)~\cite{fur2017standard} uses the term ‘‘data protection goals’’ to describe certain categories of requirements derived from data protection law.
% These requirements are aimed at properties of lawful processing operations, which have to be ensured by technical and organisational measures.
% The SDM specifies six protection goals of data protection as follows:
% % which are Data minimization, Integrity, Availability, Confidentiality, Transparency, Unlinkability and Intervenability. 
% % These protection goals reflect the protection objectives in information security that have been tried and tested in practice for many years. 
% % The objectives of availability, integrity and confidentiality thus also serve to guarantee information security in public authorities and companies, i. e. to secure and protect the data of an organisation.
% % It presents the perspective of the data subject whose rights are at stake. 
% % The protection goals Integrity, Availability, Confidentiality, Transparency, and Data Minimisation can be found conceptually in the regulation text while also referring to IT security requirements. Unlinkability and Intervenability have been adopted as data protection goals in numerous individual articles of the GDPR, among other things, via the principle of purpose limitation, erasure, and data portability.

% \begin{enumerate}[{G}1.]
% % \item \textit{\textbf{Data minimization}} covers the fundamental requirement under data protection law to limit the processing of personal data to what is appropriate, substantial and necessary for the purpose. 

% \item \textit{\textbf{Confidentiality}} refers to the requirement that no person is allowed to access personal data without authorisation.

% \item \textit{\textbf{Integrity}} refers, on the one hand, to the requirement that information technology processes and systems continuously comply with the specifications that have been determined for the execution of their intended functions. On the other hand, integrity means that the data to be processed remain intact, complete, and up-to-date.

% \item \textit{\textbf{Availability}} is the requirement that personal data must be available and can be used properly in the intended process. Thus, the data must be accessible to authorised parties and the methods intended for their processing must be applied.

% \item \textit{\textbf{Unlinkability $\&$ Data minimization}} where the \emph{unlinkability} goal refers to the requirement that data shall be processed and analysed only for the purpose for which they were collected, while the \emph{data minimization} goal covers the fundamental requirement under data protection law to limit the processing of personal data to what is appropriate, substantial and necessary for the purpose. 

% \item \textit{\textbf{Transparency}} refers to the requirement that the data subject as well as the system operators and the competent supervisory authorities can identify to a varying extent, which data are collected and processed for a particular purpose, and which systems and processes are used for this purpose, where the data flow to which purpose, and who is legally responsible for the data and systems in the various phases of data processing.

% \item \textit{\textbf{Intervenability}} refers to the requirement that the data subjects are effectively granted the right to notification, information, rectification, blocking and erasure at any time.

% \end{enumerate}
% ---------------

==> Removed/Methodology-removed.tex <==
\section{Overview of the Proposed Multi-Stakeholder Risk Assessment }\label{sec:methodology}
In this section, we summarize the methodology that we presented above. The multi-stakeholder risk assessment methodology is illustrated in Figure~\ref{fig:methodology} and consists of two main phases: (i) Mappings and Associations, and (ii) Risk Impact Assessment and Optimization. 
This figure shows all the mapping (e.g., threats to protection goals) and operation processes, as well as input/output documents. There are also reference tags associated with these processes and documents that point to equations, tables, and figures in the paper that are referenced.


% ------------------------------OLD VERSION------------------------
% This section and the following two sections present a way to define $m(T)$ and $i_s(T)$ as required by the statement of problem~\eqref{eq:msrmp}.
% The multi-stakeholder risk assessment methodology is illustrated in Figure~\ref{fig:methodology} consists of two main phases: Mappings and Associations, Risk Impact Assessment and Optimization.
% This figure shows all the mapping (e.g., threats to protection goals) and operation processes, as well as input/output documents. There are also reference tags associated with these processes and documents that point to equations, tables, and figures in the paper that are referenced.
% -------------------------------------------
% The methodology consists of two main phases: Risk Impact Assessment, and Optimization which is illustrated in Figure~\ref{fig:methodology}.
\begin{figure}[!t]
    \centering
	\includegraphics[width=0.95\textwidth]{Figures/RefinedVersion.pdf}
    \caption{Process view of the proposed multi-stakeholder risk assessment methodology}
    \label{fig:methodology}
\end{figure}

According to the figure and as described earlier, our methodology requires three inputs artifacts, namely a set of \emph{Threats}, a family $\{\mathcal{C_T}\}_{T \in \mathcal{T}}$ of \emph{Controls}, and a set $\mathcal{G}$ of data \emph{Protection Goals}. 
% In the literature there exist several approaches that deal with threat identification process and proposed potential mitigation controls.
% The decision to select a method depends on the defined project’s needs and specific concerns~\cite{shevchenko2018threat}. Indeed, the best model for your requirements is determined by the kind of threats you are attempting to model and the purpose for which you are doing so.
% For instance, Microsoft STRIDE~\cite{shostack2014threat} is a well-established threat modeling to identify security threat types. 
% It is an acronym for \emph{Spoofing, Tampering, Repudiation, Information Disclosure, Denial of Service, }and \emph{Elevation of privilege}. 
% These threats are the opposite of the primary security properties: authentication, integrity, non-repudiation, confidentiality, availability, and authorization. 
% LINDDUN is another well-known threat modeling to identify privacy threats in the system, and it stands for \emph{Linkability, Identifiability, Non-repudiation, Unawareness, Detectability, Disclosure of information,} and \emph{Non-compliance}. 
% For the sake of simplicity, and as threat input for the running example, Table~\ref{tab:threat-table} shows five possible threat scenarios relevant to our scenario. 

Security and privacy controls are the administrative, technical, and physical safeguards or countermeasures to avoid, detect, counteract, or mitigate security and privacy risks within an organization~\cite{ref_35,force2018risk}.
To establish and extract the required controls inside a system, there are several frameworks, guidelines, and best practices.
For example, NIST Special Publication 800-53~\cite{draft2017security} on Security and Privacy Controls for Information Systems and Organizations is the specification of privacy and security controls for public offices in the United States. 
It includes a wide collection of predefined controls, as well as appendices that demonstrate how to select controls that respond to different risk levels.
We have listed the security and privacy controls associated to the threat list in our scenario. 
For instance, for the \emph{unlimited data storage} threat ($T1$) in Table~\ref{tab:threat-table}, we associate some possible controls such as \emph{the purpose specification, ensuring limited data processing, ensuring data minimization}, and \emph{implementing data deletion mechanisms}. 
While for the \emph{Denial of Service} threat ($T4$), possible associated controls can be \emph{enabling off-line authentication, network monitoring}, and \emph{implementing the preventing DoS attack mechanisms like firewalls, IDS, etc}. In the following, in Table~\ref{tab:threat-control}, the complete association is provided.  

The first phase mainly focuses on the mapping processes where the output of each mapping will be used for the following processes. This phase requires the risk analyst interaction to provide the needed inputs for the second phase. For instance, the first process that needs to be taken into account in this phase is to determine \textit{stakeholders} and their impact \textit{preferences} and assign a \textit{weight} to each of them. The second phase will be fully automated, where  \textit{Impact Level Evaluation} and \textit{Threat Criticality Quantification} processes will use the outcomes obtained from the previous phase to generate a list of Pareto-Optimal solutions as final output. In the following two sections, we describe each phase in detail.


% \begin{figure}[!t]
%     \centering
% 	\includegraphics[width=0.95\textwidth]{Figures/Reference Eqs-Tables.pdf}
%     \caption{Data flow of the proposed methodology}
%     \label{fig:reference}
% \end{figure}
% In Figure~\ref{fig:reference}, we have sketched all the artifacts and their relations with the intention of providing a comprehensive picture of the data flow in the proposed methodology. It illustrates the mapping relations between the artifacts, the output of each mapping, the operations (i.e., the multiplication operation), and the reference tags to the equations and tables.
% In this figure, artifacts are divided into two categories, external and internal. External artifacts are those that are used as input data, where internal artifacts are those that must be specified by the data controller, which are the involved stakeholders, their preferences, and the weights assigned to those preferences.

%  External artifacts are taken from outside which are a list of threats, goals, and controls. 
% \subsection{\textbf{Threat Modeling}}


% \subsection{\textbf{Impact Assessment}}

%  Generic approach for RISK IMPACT ASSESSMENT 

% Generic setting of methodology 

==> Removed/Optimization.tex <==
\section{Risk Assessment and Optimization}\label{sec:optimization}
In this phase of the methodology, using the outputs from the previous phase, we first evaluate the impact levels for each stakeholder (i.e., $i_s(T)$) and then quantify the criticality level of each threat. After that, the risk exposure levels will be calculated, resulting in a list of risk levels for each stakeholder. The Pareto-Optimal algorithm is then applied to the obtained list in order to find the optimal solutions. In the following, each of these processes is explained in detail.

% As we discussed in the problem definition section (Section~\ref{sec:MSRToAP}), our methodology’s ultimate goal is to solve a multi-objective problem by finding an RMP to minimize risk levels for all involved stakeholders in a given system. 

% Up to this phase of the methodology, we have proposed a method to define \emph{how} the impact has to be evaluated for each stakeholder when the existing threats are known. However, as we discussed in the problem definition section (Section~\ref{sec:MSRToAP}), our methodology’s ultimate goal is to solve a multi-objective problem by finding an RMP to minimize risk levels for all involved stakeholders in a given system. Hence, in this section, we focus on the optimization process, which is the last phase of our methodology.  

\subsection{\textbf{Impact Level Evaluation}}~
By having the obtained values from the \textit{threat-preference association} process and the \textit{weight} assigned to each preference, each threat's impact level is evaluated. 
We have assigned a weight to each preference (PW), as can be seen in Table~\ref{tab:threat-preference-association}. For example, the data subject's \emph{health condition} has the highest weight among all of the data subject's preferences, where the greatest weight from the data controller point of view is \emph{financial situation}. It is worth restating that the reason for using such a cross-weighting method is to decrease the level of subjectivity in the assessment.
The computed impact levels will be used as one of the inputs for the risk calculation process.
Formula~~\ref{eq:threatImpact} computes the impact level of each threat for each stakeholder.
\begin{equation} \label{eq:threatImpact} 
   i_s(T)= \sum_{\substack {p\in \mathcal{P}\\ }} IV_{(T,p)}^{s} ~\times ~ PW_{p}^{s}
\end{equation}
In this formula, 
% $n$ is the number of preferences a stakeholder has, as well as, 
$IV_{(T,p)}^{s}$ represents the impact value of threat $T$ for preference $p$ from the point of view of stakeholder $s$, and $PW_{P}^{s}$ is the assigned weight to that preference. 
For example, according to Table~\ref{tab:threat-preference-association}, the impact value of the \textit{health condition} for the second threat ($T2$) is 4, and the impact level for $T2$ from data subject standpoint equals:~$i_{DS}(T2)=\frac{(0.4 \times 4)+(0.2 \times 2)+(0.3 \times 2)+(0.1 \times 3)}{4}=0.725$.
In Table~\ref{tab:risk-goals} (the third column), we have evaluated and reported the normalized impact levels (by using the assigned impact levels in Table~\ref{tab:threat-preference-association}) for each threat from two points of view.


% As can be seen in Table~\ref{tab:threat-preference-association}, we have assigned a weight to each preference. For instance, for the data subject, the health condition has the highest weight among all the data subject’s preferences. 
% As the same performed for the threat criticality, the obtained impact from formula~\ref{eq:threatImpact} is normalized in order to evaluate the actual impact for each goal.
% \begin{align} 
% \forall _{i=1,...,t} \: ImpactT_{i}^{s}= \sum_{j=1}^{n} I_{(i,j)}^{s_{}} \times APW_{(i,j)}^{s}
% \label{eq:threatImpact} 
% \end{align}



% In Table~\ref{tab:risk-goals}, the overall normalized impact levels are presented for each threat and stakeholder separately. 
\subsection{\textbf{Threat Criticality Quantification}}
The purpose of threat criticality ($TC$) is to quantify the seriousness of each threat. We use a simple technique to evaluate $TC$ based on the relationship between the protection goals and the identified controls for each threat. 
% For the processing of the risk impact assessment, the value of $TC$ is necessary.
To quantify the threat criticality value for each threat, two values must be considered, (i) the observation weight ($OW$), and (ii) the threat evidence ($TE$). Basically, the threat criticality shows the level of danger of a threat among all threats.
% The observation weight for each threat is measured in table~\ref{tab:combined-table}.
The threat criticality computes by Formula~\ref{eq:Sc} to determine how much a threat has precedence over the other threats. 
% In this formula, $OW_{T}$ represents the value of the observation weight for threat $T$, and $TE_T$ represents the evidence value of the existence of the threat $T$, which is a value in (0...1].
% The TE value expresses the system's capability in being able to mitigate the threat, and this value comes from the degree of implementation controls for the threat. The more defined controls being implemented for the threat, the less TE value will have for it and vice versa.  
% For simplicity, in our scenario, we consider these values \{$0.4, 0.35, 0.25, 0.83, 0.66$\} as threat existence values to the threats \{$T1, T2, T3, T4, T5$\}, respectively.
% For simplicity, for now we consider this value for each threat equals $1$, which means the associated controls for threats are not implemented at all. 
% In the next section, we will explain in detail how to calculate the threat existence value.

\begin{equation} \label{eq:Sc}  
    \forall_{T=1,..,t} \, \: TC_{T}= OW_{{T}} \times TE_{T} 
\end{equation}
\begin{equation} \label{eq:RSP}
 \forall_{T=1,..,t} \, \: 
 NTC_{T}=\frac{TC_{T}}{\sum_{j=1}^{t}TC_{j}}
\end{equation}

% Indeed, the \textit{TC} indicates how much a threat can be severe.
% To calculate risk exposure, we need to normalize the obtained values through Formula~\ref{eq:RSP}.
% \subsection{\textbf{Risk calculation}}
% As can be seen in Figure~\ref{fig:methodology}, three inputs need for the risk calculation process, the threat criticality and impact level values which computed in the previous phase, and the feasible set. 

\begin{table}[!b] \center
        \caption{Normalized threat criticality and impact level values together with the computed protection goals' risk impacts for each threat for the data subject (DS) and the data controller (DC).} \label{tab:risk-goals}
	    \includegraphics[width=0.99\textwidth]{Figures/Risk-Result.pdf}
\end{table} 


% Indeed, the \textit{TC} indicates how much a threat can be severe. 
We then normalize the obtained values through Formula~\ref{eq:RSP} to calculate risk exposures. 
The normalized threat criticality values for each threat in our scenario by using the obtained observation weights (Table~\ref{tab:Threat-Goals}) and the calculated $TE$ values (Table~\ref{tab:threat-control}) are reported in the second column of Table~\ref{tab:risk-goals}.
% and in the third column, the normalized impact levels are reported (by using the assigned impact levels in Table~\ref{tab:threat-preference-association} and computing through Formula~\ref{eq:threatImpact}) for each threat for both stakeholders.
\subsection{\textbf{Risk Calculation}}
After obtaining the two values from two previous processes, we calculate the risk levels through Formula~\ref{eq:risk-exposure} for each stakeholder in terms of how much the protection goals are at risk. Then by aggregating them, the final risk levels or, in other words, the obtained objective functions from a multi-objective point of view.
% By obtaining and normalizing the two values above (the threat criticality and impact levels),

\begin{equation} \label{eq:risk-exposure}
    	GoalRA_{G}^{S}= \frac{ ~\sum_{T=1}^{t}(if~T~compromises~G~then) ~NTC_{T} \times i_s(T)}{X_{G}}
\end{equation} 
% 	\forall _{G=1,..,g} ,\,\:
% 	GoalRA_{G}^{S}= \frac{\sum_{T=1}^{t}TC_{T}\times ImpactLevel_{T}^{S} }  {X_{G}}
In this formula, $X_{G}$ represents the total number of affection of the goal $G$ by threats, in another word, how many threats affect the goal $G$. For instance, according to Table~\ref{tab:Threat-Goals} the \textit{intervenability} goal ($G6$) is affected only by $T5$ which means $X_{G6}$ is 1. As an instance of the risk calculation process, we have reported the risk exposure results in Table~\ref{tab:risk-goals} for the case of when $TE$ values are the ones reported in Table~\ref{tab:threat-control}. 
% The risk average is computed for each goal for both stakeholders in Table~\ref{tab:risk-goals}. 
For example, according to Table~\ref{tab:risk-goals}, the risk average of \emph{confidentiality} goal ($G1$) for the data subject is $0.074$, while this value for the data controller is $0.087$. 
Notice that since the \emph{transparency} goal ($G5$) is not affected by non of the threats (according to Table~\ref{tab:Threat-Goals}), it is not mentioned in Table~\ref{tab:risk-goals} neither use for the risk calculation process.
By aggregating the risk average of protection goals, the overall risk from the data subject’s point of view is $0.549$, and it is $0.576$ for the data controller. 

As it is depicted in Figure~\ref{fig:methodology}, the output of the risk calculation process will be a list of risk levels which are the objective functions for our multi-objective optimization problem. In the next process, we apply Pareto-Optimal notion to solve this problem and find optimal solutions.



% \subsection{\textbf{Multi-Objective Optimization Problem}}


%  Therefore, to solve a multi-objective problem using classical methods would not
% \subsection{\textbf{Optimizing MSRToAPs}}




% \subsection{Risk management policy}
% A risk management policy (RMP) is considered as a set of technical and organizational measures to deal with risk. 
% In a multi-stakeholder risk assessment, different stakeholders have different preferences to assess the potential impact of threats. Thus, the selected RMP has different effects on the stakeholders' risk exposure. 
% Therefore, the purpose of a selected RMP is to minimize the risks for all the considered stakeholders while taking into account, at the same time, additional constraints, such as legal prescriptions or business requirements.
% % Indeed, the MSRToAP is defined as the problem of finding an optimal RMP among a list of candidate RMPs that simultaneously minimize the risk exposure for all stakeholders.
% However, finding an optimal RMP considers as the multi-objective optimization problems, where to solve them requires optimizing at least two different functions (objectives), which in case of MSRToAP, minimizing the risk exposure for all stakeholders. The searched optimum of these problems is not a single solution as in the mono-objective case, but a set of solutions known as the Pareto optimal set. Any element in the optimal set is no better than the other ones for all the objectives. The optimal-set is given to the decision-maker, who has to choose the best trade-off solution corresponding to his/her preferences.




% \subsection{\textbf{Generating Pareto-optimal Solutions for an MSRToAP}}

% \subsection{\textbf{Risk Calculation}}
% This process is the same as the previous phase that we calculate the risk levels through Formula~\ref{eq:risk-exposure}. 
% As shown in Figure~\ref{fig:methodology}, three inputs need for the risk calculation process: the computed impact level values, the observation weights, and threat evidence values that extract from the feasible set. Therefore, the obtained feasible set is used to calculate the threat criticality values ($TC$s).


% By formula~\ref{eq:risk-exposure}, we can calculate the risk exposure from different perspectives for each protection goal. In this formula, $X_j$ is the total number of affection of the $j$-th goal by threats, or other words, how many threats affect the $j$-th goal. For instance, according to table~\ref{tab:Threat-Goals} the \textit{intervenability} goal has affected one time (out of five) which means $X_5$ is 1.

% \begin{align} \label{eq:risk-exposure}
% 	\forall _{j=1,..,g} ,\,GoalImpact_{j}^{S}= \frac{\sum_{i=1}^{t}NTC_{i}\times ImpactT_{T}^{S} }  {X_{j}}
% \end{align}

% \begin{figure}[!t]\center
% 		\includegraphics[width=0.97\textwidth]{Figures/Risk-Goal-Level.pdf}
% 		\caption{The risk exposures for data subject and data controller based on protection goals in the running example.} \label{risk-goals}
% \end{figure}
% Proposing an efficient method to discover all Pareto-optimal solutions in an MSRToAP, then we finding the Pareto-optimal solutions.

\subsection{\textbf{Finding Pareto Optimal Solutions}}
% multi-objective part
As we mentioned earlier, MSRMP is considered as the problem of finding an RMP to minimize the risk exposures for all associated stakeholders in the risk assessment procedure.
The presence of multi-objective in a problem, produce a list of optimal solutions which are Pareto-optimal solutions, rather than a single optimal solution. 
Therefore, searching for a solution and selecting as the final solution (ideally from non-dominated solutions) in an MSRMP must be done in two steps. 
The first step is to discover Pareto-optimal solutions by using or designing an optimization algorithm to generate all non-dominated solutions. However, by having this solution set, it cannot be assumed one solution better than other optimal solutions without any additional information.
Thus, the second step is to propose a methodology to choose a single solution from the set of Pareto-optimal solutions, while taking into account the preferences of the decision-maker.
In this paper, we mainly focus on the first step to propose a method to generate all possible Pareto-optimal solutions in an MSRMP.
% 

After generating the feasible solutions set and then calculating the risk exposures based on this set, the next step is to find Pareto optimal solutions over this set. As we described earlier, based on Pareto optimality definition, finding solutions can be defined as to find a vector of objective functions $x$, which optimizes a vector of $M$ objective functions $f_i(x)$ where $i=1,2,...,M$, and $M$ is the size of feasible set. Basically, for an MSRMP, we intend to minimize $f_i$ where $i=1,2,...,M$. An objective function vector $x$ is said to dominate an objective function vector $y$ (also written $x \prec  y$) if and only if their objective vectors $f_i(x)$ and $f_i(y)$ satisfies: 
\begin{align} 
\begin{split}
f_i(x) \leq f_i(y) \, \forall _i \in \, \{1,2,...,M\} ;and \\ 
\exists _i \in \{1,2,...,M\}|f_i(x) < f_i(y)
\end{split}
\label{eq:Pareto} 
\end{align}
All objective function vectors that are not dominated by any other objective function vectors are considered to build the Pareto optimal set. After discovering this set, the decision-maker will choose a solution based on his/her preferences. This process is called decision making, which is the last process of our proposed methodology.
% In this paper, we have not a plan to propose a methodology only for the decision making process, however, in the following we have
% and in the following, we will propose a methodology to assist the decision-maker to select a solution among the optimal set.

\subsection{\textbf{Decision-Making}}
The final solution of a MOOP obtains from the decision-making process. 
The integration of the decision-making process with the optimization process must allow for the identification of a single solution that is highly compatible with the decision maker's preferences among the Pareto-optimal solutions generated by the optimization procedure.
The way how the search and the decision processes are jointed can be categorized into three different groups of methods~\cite{kaliszewski2006soft} as follows: 
\begin{enumerate}[I.]
\item \textbf{Priori methods}: In these methods, before applying the optimization process, the decision-maker must determine her/his preferences. The determined preferences are defined as an aggregate function that merges individual objective values into a single utility value. 
\item \textbf{Posteriori methods}: The Pareto-optimal without considering the decision-maker preferences is generated, then he/she chooses the most favored one between the alternatives.  
\item \textbf{Interactive methods}: In these methods, both processes are performed simultaneously. At each step, partial preference info is applied by the decision-maker. In the optimization process, the algorithm applies this info to produce better solutions with respect to the info received from the decision-maker.
\end{enumerate}
In our methodology, after finding the Pareto-optimal solutions, the decision maker choose a solution as  the optimal solution which can be considered as a posteriori method.
% In this paper, after finding the Pareto-optimal solutions, we intend to propose a method for decision making process which can be considered as a posteriori method.
% \subsection{Proposed decision making method}



% According to computational complexity of MSRToAP


% \subsection{Computational Complexity of MSRToAP}
% The goal of computational complexity is to classify problems, and the complexity of a problem is the infimum of the complexities of the algorithms that may tackle the problem. Thus the complexity of a problem would not be higher than the complexity of any algorithm that intends to solve it.
% The complexity of MSRToAP is $O(m^N)$, where $N$ represents the number of variables (population size), which are security and privacy controls, and $m$ is the number of possible values that can be assigned to each control as implementation status. 
% In case of MSRToAP, the implementation value can be one of these statuses not implemented, or partially, or fully implemented, which means $m$ equals three.
% However, the global complexity is exponential, and the worst-case time complexity for MSRToAP is $O(3^N)$. Therefore, MSRToAP settles in the exponential-time complexity class with high computational complexity, which is very expensive in case of large population sizes.
% Indeed, the complexity time of MSRToAP is the time of computing all possible solutions without considering the computation time required to find the optimal solutions. 
% In this situation, using the reduction concept is a good practice to define the problem into another problem, which can be reduced from exponential-time to low computational time, e.g., to polynomial time.


% The classical optimization technique broadly recommends that the multi-objective problem transforms into a single-objective optimization problem by emphasizing one particular Pareto-optimal solution at a time. 
% Using these kinds of techniques to discover various solutions, demanded to be applied many times, optimistically capturing a different solution in each run of the algorithm~\cite{deb2000fast}.

% \subsection{Evolutionary Algorithms}
% Evolutionary algorithms (EAs) are a subclass of Evolutionary Computation and belong to a set of general stochastic search algorithms. EAs apply where optimal decisions require to be adopted in the presence of trade-offs between multiple objectives. EAs are extremely appealing for multi-objective optimization analysis in comparison to classical optimization methods. In the context of multi-objective optimization, numerous multi-objective evolutionary algorithms (MOEAs) have been proposed.
% The essential explanation behind the MOEAs is their capability to discover multiple Pareto-optimal solutions in one single run. 
% One of the primary goals of MOOP solvers is to obtain a set of non-dominated solutions with the minimum distance to Pareto-front; on the other hand, evolutionary algorithms can produce these sets in each generation. Therefore, EAs are well suited to solve MOOPs.
% \subsection{MOEA Techniques}
% A Variety of techniques are available in the context of multi-objective evolutionary algorithms. In~\cite{deb2001multi} and~\cite{coello2007evolutionary} both have discussed various MOEAs in their book to express the difference in the framework and operators of these MOEAs. 
% Some examples of MOEAs are: vector evaluated genetic algorithm (VEGA), indicator-based evolutionary algorithm (IBEA), epsilon multi-objective evolutionary algorithm (epsilon-MOEA), Pareto archived evolution strategy (PAES), and multi-objective evolutionary algorithm based on decomposition (MOEAD).
% However, the most representative, discussed and reviewed are multi-objective particle swarm optimizer (MOPSO), strength Pareto evolutionary algorithm (SPEA) and the improved version of it (SPEA2), Pareto envelope-based selection algorithm (PESA), non-dominated sorting algorithm (NSGA) and the second version of it (NSGA-II). 
% Knowing and selecting which algorithm has the best performance among various MOEAs is a common challenge for most scientists and researchers.
% Extensive comparison studies and numerical simulation on various test problems demonstrate a superior overall behavior of NSGA-II and SPEA2 compared to other algorithms~\cite{konak2006multi,yu2018evaluating}.
% In cases with two objectives, NSGA-II has shown better results than SPEA2; in contrast, for more than two objectives, SPEA2 seems to indicate some advantages over NSGA-II. 


% \subsection{Non-dominated Sorting Genetic Algorithm (NSGA)}
% In 1994, Srinivas and Deb~\cite{srinivas1994muiltiobjective} proposed one of the first EAs which named non-dominated sorting genetic algorithm (NSGA). Over the years, it turned out that the NSGA approach had some drawbacks that the authors decided to modify and improve it. These drawbacks were:
% \begin{itemize}
% \item High computational complexity of non-dominated sorting, it was $O(MN^3)$ where $M$ is the number of objectives and $N$ is the population size.
% \item Lack of elitism, which has proved approaches with elitism, can speed up the performance of the genetic algorithm significantly; furthermore, it helps to prevent the loss of good solutions.
% \item Need for specifying the sharing parameter~\cite{deb2000fast,deb2001multi}. 
% \end{itemize}

% In NSGA-II~\cite{deb2000fast} all the mentioned drawbacks have eliminated, and in terms of computational complexity by applying a proper book-keeping strategy, the complexity reduced to $O(MN^2)$. 
% On the other hand, a fast non-dominated sorting approach, rapid crowded distance estimation procedure, and simple crowded comparison operator are the distinctive characteristics of NSGA-II, made it one of the most popular multi-objective optimization algorithms.


% \section{Discussion}
% In this section we intend to propose the solution in which we can solve MSRToAP.
% In order to solve MSRToAP, we 

% \begin{figure}[t]\center
% 		\includegraphics[width=\textwidth]{Figures/ProblemEncoding.pdf}
% 		\caption{MSRToAP encoding} \label{ProblemEncoding}
% \end{figure}

% To solve MSRToAP instances, the authors~\cite{mollaeefar2020} proposed an automated technique. 
% The proposed technique has the objective of illustrating \textit{how} the impact has to be evaluated for each stakeholder when the existing threats are identified.
% It comprises of two primary stages: (i) configuration stage, where the characteristics of the specific organization are captured and transformed into parameters of the risk evaluation method; and (ii) execution stage, in which the identified threats are estimated based on the controls, and their impact level evaluated, which in turn defines the risk exposure for the various stakeholders. 

% \section{Multi-Stakeholder Risk Trade-off Analysis Problem}

% The General Data Protection Regulation (GDPR) has been presented to guarantee European citizens' fundamental rights concerning personal data protection and privacy. One of the primary objectives of the GDPR is to give individuals control over their data. Controllers and processors of personal data must provide appropriate technical and organizational measures to minimize the risks that personal data can be abused, for instance, in the case of a data breach.  On the other hand, to evaluate the adopted security and privacy measures and minimize the impact of them on the rights and freedom of individuals, GDPR prescribes to perform a Data Protection Impact Assessment (DPIA). This kind of assessment differs from classical risk analyses in which the actor carrying out the evaluation is also interested in diminishing its risk. Protection of data subjects' rights may cause conflict with organizations' objectives where organizations shall provide adequate security measures while struggling with various types of constraints (e.g., budget). The Multi-Stakeholder Risk Trade-off Analysis Problem (MSRToAP) has been introduced~\cite{mollaeefar2020} to alleviate the problem of conflicts of interests and help data controllers make more informed decisions about which security mechanisms allow for a better trade-off between their requirements and those of the data subjects.

==> Removed/Pseudocode.tex <==


\begin{lstlisting}
/**
Assumptions: 
1) A Solution object constituted of two double values (x,y) where represent the value of "oir" each stakeholder.
2) The size of feasible set is computed.
**/
List<Solution> final_Solutions = new ArrayList<>(); // Define a final list of solutions
List<Solution> temp = new ArrayList<>(); // Define a temporary list
int feasible_Set_Size; // Compute the size of feasible set
int counter=0; // Define a variable for counting the number of generated solutions
int d; // Define a variable to generate solution list for each iteration
boolean check = true;
while(check)
	{   
      //Generate a list of solutions with size of d and adding to the temp list
		temp.addAll(final_Solutions); // Adding also all discovered Pareto Solutions up to now to temp
		final_Solutions.clear(); // Clearing final_Solutions to add Pareto Solutions based on the new iteration
            for (Solution a : temp) { // Apply Pareto-Optimality definition on the temp list
                boolean flag = false;
                for (Solution b : temp) {
                    if (a != b) {
                        if (a.getX() >= b.getX() && a.getY() >= b.getY()) {
                            flag = true;
                        }
                    }
                    if (flag)
                        break;
                }
                if (!flag)
                    final_Solutions.add(a); // Adding a solution as Pareto solution
            }
            counter+= d;
            temp.clear();
            if (counter >= feasible_Set_Size) { // Checking size of the generated solutions
                check = false;
            }
    }
return final_Solutions; // Return the final Pareto solution list
\end{lstlisting}


==> Removed/RedComment.tex <==
\textcolor{red}{SILVIO HOW ABOUT ADDING THIS AT BEGINNING OF SECTION 4.2.\\
In the above, we evaluated the impact levels only on the basis of the assumption that all threats have an equal importance level (apart from the mitigation controls that state their presence). 
Additionally to the above assumption, we must consider the fact that the aversion level association is a subjective task. 
Many factors can be considered to determine the importance level of a threat, and a threat may be classified as an importance threat based on certain characteristics of the data itself, such as the data type sensitivity, the data volume, the data retention period, etc.
\\ THIS COULD BE EXTENDED...
}

\textcolor{blue}{
This way may become too subjective if only impact levels (i.e., the level of aversion in Table~\ref{tab:threat-preference-association}) are going to be considered. By defining one further association for threats, we are able to evaluate and then prioritize them. As a consequence of this association (i.e., threat-protection goal association in Table~\ref{tab:Threat-Goals}), the subjectivity level of the methodology will reduce. Consider the following instances to illustrate the distinction between these two associations:
\begin{itemize}
    \item (i) where according to Table~\ref{tab:Threat-Goals}, threat $T_5$ has impacted on only one protection goal (i.e., $G6$). However, according to Table~\ref{tab:threat-preference-association}, $T_5$ is the most significant threat from the data subject point of view with a high aversion level.
    \item (ii) where according to Table~\ref{tab:threat-preference-association}, threat $T_3$ has the high aversion level to compare with other threats from the data controller point of view, while the aversion level for the data subject is even less than $T_2$ and $T_5$. However, according to Table~\ref{tab:Threat-Goals}, threat $T_3$ is the most dangerous threat by affecting three protection goals. Whereas in this table, $T_1$, $T_3$, and $T_4$ are impacting on two protection goals.
\end{itemize}
Therefore, combining these two associations helps us have a less subjective impact assessment.
}

==> Removed/Removed.tex <==
% Section 4
% ----Risk Definition
Risk is traditionally interpreted as R = L $\times$ I, where \textit{“L”} is the probability of happening the risky events, and \textit{“I”} is their negative impact on individuals, assets, and organizational goals if they happen. We move from the idea that, within the same accountability context (i.e., the scope, for which the same stakeholder is the accountant for the risk management), different stakeholders are exposed to different risks. However, essentially only one of them is responsible for conducting the risk analysis and applying the proper measures. This is significantly clarified in laws and regulations, such as GDPR, so that a particular subject (the data controller (dc)) is accountable for the risks related to the data processing activities it offers, but the risk assessment must be carried out from the perspective and the interest of the data subject (ds).
Given these hypotheses, we redefine risk as $R =$ $\langle$ $R_{ds}, R_{dc} $ $\rangle$ $=$ $\langle$ $(L_{ds} \times I_{ds}),(L_{dc} \times I_{dc})$ $\rangle$. 

From the aforementioned distinction between \textit{accountability} and \textit{interest}, we derive one further property: 
since the interested parties are many, the perceived impact is different for each party;
on the other hand, since the accountable stakeholder is one by definition, the estimation of the likelihood is the same for all the stakeholders.
We assume therefore that $L_{ds}$ = $L_{dc}$, and the risk becomes $R = $ $\langle$ $(L \times I_{ds}), (L \times I_{dc})$ $\rangle$.
Since there are lots of risk assessment approaches in the literature that cope with the likelihood estimation and that its actual value is irrelevant for the purpose of comparing the risk exposures, we focus on the estimation of the impact levels.
Hence, the risk exposure depends on two things: (i) the method adopted to estimate the potential impact of threats on each stakeholder; and (ii) the threats associated with the system configuration.
In the following, we propose a multi-stakeholder cybersecurity risk assessment methodology which is an extended and refined version of our previous proposed methodology~\cite{mollaeefar2020}.

% -----------Removed Figure and its definition
\begin{figure}[!t]
    \centering
	\includegraphics[width=0.95\textwidth]{Figures/Reference Eqs-Tables.pdf}
    \caption{Data flow of the proposed methodology}
    \label{fig:reference}
\end{figure}


In Figure~\ref{fig:reference}, we have sketched all the artifacts and their relations with the intention of providing a comprehensive picture of the data flow in the proposed methodology. It illustrates the mapping relations between the artifacts, the output of each mapping, the operations (i.e., the multiplication operation), and the reference tags to the equations and tables.
In this figure, artifacts are divided into two categories, external and internal. External artifacts are those that are used as input data, where internal artifacts are those that must be specified by the data controller, which are the involved stakeholders, their preferences, and the weights assigned to those preferences.
% ---------------



\section{Threat Modeling}\label{sec:threat-modeling}
Threat modeling has a vital role in building a secure software system by considering how an adversary might compromise the system.
Indeed, it supports understanding security and privacy threats in a given system, how those threats impact data subjects and the organization as the data controller and identifying possible security and privacy countermeasures to mitigate potential attacks.
It is highly recommended to apply threat modeling early in the development cycle, where potential issues can be detected early and remedied to prevent possible later consequences.
There are several approaches that may be used while undertaking threat modeling, such as Microsoft STRIDE~\cite{shostack2014threat}, PASTA~\cite{ucedavelez2015risk}, LINDDUN~\cite{wuyts2015linddun}, and Trike~\cite{saitta2005trike}. Each threat modeling technique follows a somewhat different set of phases.
Not all methods are comprehensive, or in other words, a particular threat modeling method is not suggested over the others. The decision to select a method depends on the defined project’s needs and specific concerns~\cite{shevchenko2018threat}. Indeed, the best model for your requirements is determined by the kind of threats you are attempting to model and the purpose for which you are doing so.
% However, our methodology’s threat modeling phase is roughly the same as other threat modeling methods in terms of the processes that need to be performed. 
Our objectives of conducting this phase are: (i) to have a comprehensive understanding of the system that supports security and privacy-aware specification of the data processing, (ii) to identify potential threat scenarios, and then (iii) to determine countermeasure controls according to the identified threats. In this phase, the following steps require to be fulfilled:

% Our threat modeling phase is almost the same as other threats modeling in terms of the processes that need to be done, with this objective to have a comprehensive understanding of the system, identifying potential threat scenarios, and determining countermeasure controls. In this phase, the following processes require to be fulfilled:

\subsection{\textbf{Security and privacy-aware specification of the data processing}}
\begin{figure} [!t]
    \centering
	\includegraphics[width=0.95\textwidth]{Figures/DFD_ACME.pdf}
    \caption{High-level data flow diagram in our eHealth scenario.}
    \label{fig:DFD}
\end{figure}

Security by Design (SbD) and Privacy by Design (PbD) are principles increasingly identified as necessary for dealing with design faults that may jeopardize security or privacy in the system~\cite{alshammari2017}. 
Furthermore, their application is also envisaged by the GDPR, as it demands Data Protection by Design (DPbD) for any systems that involve personal data in their processing.

[THIS SECTION NEEDS TO BE EXTENDED AND REFINED]

The first step of threat modeling aims to characterize a system in such a comprehensive and detailed way that potential security and privacy threats can be found. 
In this step, all the assets and the main actors involved in the system must be identified.
For example, Figure~\ref{fig:scenario} depicts the main actors and their interactions with the system's components in our scenario. At the client-side (End-user), the Mobile Health App dynamically receives the biometric data from the smart health device, which is worn/used by the patient. Then the data is transferred to the HCare-web server (Application provider) for further processing. After receiving any updates (such as biometric data or user requests) from the patients, the doctors monitor their health condition at the health service provider side. Through the HCare-web, doctors can write a prescription, respond to requests, initiate a medical alert, etc. 

In this step, the data flow diagram (DFD) aids represent how data flow through the system and handled by different sub-processes. A DFD presents a logical depiction of the system’s implementation and shows the system’s large-scale architecture. It illustrates what entities exist in implementing the system and how these entities exchange information. It is also helpful for the threat identification process to characterize how adversaries can threaten the various phases of the data flow, such as collecting, storing, using, transferring, and deleting.
For our scenario, we decided to use the DFD in Figure~\ref{fig:DFD} as the system documentation in Figure~\ref{fig:methodology}, as this helps highlight how data is modified during the data processing activity under consideration.  

% The data flow diagram of processing the health data recorded in our scenario is depicted in Figure~\ref{fig:DFD}.  

% \subsection{\textbf{Selecting threat types} }

\subsection{\textbf{Threat scenario identification}}
\begin{table}[!b] \center
    \caption{Security and privacy threat types defined in~\cite{shostack2014threat,wuyts2015linddun}}
    \includegraphics[width=0.99\textwidth]{Figures/Threat-types.pdf}
    \label{tab:threat-types}
\end{table}
A threat is a potential adverse action or event facilitated by a vulnerability that results in an undesired impact on the system. Threats usually may come from authorized users (insiders) or unauthorized users (outsiders). All the information gathered from the last phase will assist in identifying possible threats in the system.
Utilizing the provided threat lists will also help in the threat identification process by reviewing each asset, process, access point, and data flow in the system and creating threat scenarios regarding violation of security and privacy properties. 
In general, threats in a given system can be divided into two broad classes, namely security and privacy threat types. 
The identification of security and privacy threats entails knowledge of the types of threats to be identified.
High-level categories of security~\cite{hernan2006threat} or privacy~\cite{deng2011privacy} threats---which might comprise multiple sub-types of threats in a hierarchical structure---are used in threat modeling. Here, the word “categories” is sub-optimal, as it is aimed only to help in the remainder of the main types of threats.
The categories are not disjunct groups under which all the different threat types can be unambiguously placed. Rather, the many forms of threats are overlapping and dependent~\cite{sion2020}. For instance, spoofing an identity can lead to the elevation of privilege in the system. In addition to the threat modeling threat types, there are a variety of different knowledge sources on security and privacy concerns at various abstraction levels. Low-level vulnerabilities in concrete software products~\cite{cve}, design flaws~\cite{arce2014,hosseini2017,tuma2019}, architectural weakness~\cite{cwe, santos2017catalog}, and attack patterns~\cite{CAPEC} are only a few examples in this regard.

~STRIDE is a well-established threat modeling presented by Microsoft to identify security threat types. 
It is an acronym for \emph{Spoofing, Tampering, Repudiation, Information Disclosure, Denial of Service, }and \emph{Elevation of privilege}. These threats are the opposite of the primary security properties: authentication, integrity, non-repudiation, confidentiality, availability, and authorization. 
LINDDUN is another well-known threat modeling to identify privacy threats in the system, and it stands for \emph{Linkability, Identifiability, Non-repudiation, Unawareness, Detectability, Disclosure of information,} and \emph{Non-compliance}. 
These threats are the negation of privacy properties: unlinkability, anonymity and pseudonymity, plausible deniability, undetectability and unobservability, confidentiality, content awareness, policy and consent compliance. All the mentioned threats above are described in Table~\ref{tab:threat-types}. Notice that the \emph{disclosure information} is a common threat in both methods. Therefore, we do not describe it again for LINDDUN in Table~\ref{tab:threat-types}. Indeed, Table~\ref{tab:threat-types} is the content of the database in Figure~\ref{fig:methodology} called Security $\&$ Privacy threat types. It is possible to customize it depending on the scenario considered, and here, we use this for our scenario.

\begin{table}[!b] \center
    \caption{An example of possible threat scenarios and their mapped threat types in the ACME scenario}
    \includegraphics[width=0.99\textwidth]{Figures/Threat-scenarios.pdf}
    \label{tab:threat-table}
\end{table}


Each security and privacy property can be threatened by different type of threats in a given system. 
% Therefore, in this step, the potential threat scenarios must be identified. 
For the sake of simplicity, Table~\ref{tab:threat-table} shows five possible threat scenarios relevant to our scenario. This is the list of threat scenarios as derived by the threat scenario identification process in Figure~\ref{fig:methodology}, by using the database of Security $\&$ Privacy threat types (Table~\ref{tab:threat-types}) together with the system documentation in Figure~\ref{fig:methodology}, i.e., the DFD in Figure~\ref{fig:DFD}.
% Each threat is mapped to one (or more) possible threat type(s), as well as the relevant data processing principles (we will explain these principles in Section~\ref{sec:threat-principle}) taken from those listed in the GDPR and relevant approaches such as STRIDE and LINDDUN.


\subsection{\textbf{Determining security and privacy controls}}
Security and privacy controls are the administrative, technical, and physical safeguards or countermeasures to avoid, detect, counteract, or mitigate security and privacy risks within an organization~\cite{ref_35,force2018risk}.
To establish and extract the required controls inside a system, there are several frameworks, guidelines, and best practices.
For example, NIST Special Publication 800-53~\cite{draft2017security} on Security and Privacy Controls for Information Systems and Organizations is the specification of privacy and security controls for public offices in the United States. 
It includes a wide collection of predefined controls, as well as appendices that demonstrate how to select controls that respond to different risk and effect levels.

The last step of our threat modeling phase is to determine the security and privacy controls for each identified threat scenarios. 
% In our scenario, we have determined the security and privacy controls for each threat, in total twenty-five controls for five identified threat scenarios. 
We have determined and listed the security and privacy controls in our scenario. 
For instance, for the \emph{unlimited data storage} threat (T1) in Table~\ref{tab:threat-table}, we associate some possible controls such as \emph{the purpose specification, ensuring limited data processing, ensuring data minimization}, and \emph{implementing data deletion mechanisms}. 
While for the \emph{Denial of Service} threat (T4), possible associated controls can be \emph{enabling offline authentication, network monitoring}, and \emph{implementing the preventing DoS attack mechanisms like firewalls, IDS, etc}. The complete association is provided later in Table~\ref{tab:threat-control}. 

% However, due to avoid multi-time representing them, and since we need to refer to these controls in the \emph{Risk Calculation and Optimization} phase (cf. Section~\ref{sec:optimization}), therefore, we will present them all together with the threat scenarios in Table~\ref{tab:threat-control}.

% -------------Example Table 

\begin{Example}{}{} \small
%   So far we learnt from the two previous examples that 
    From Example 2, we learnt how the impact residue for each threat can be computed. Through $\mathit{ir}_s^{\mathit{avg}}(C)=\frac{1}{|\mathcal{T}|} \Sigma_{T\in \mathcal{T}}~ \mathit{ir}_s(T,C)$
    the overall impact residue can be obtained for each stakeholder. 
    % by having the derived impact residue for each subset 
    % would be as follow:
    For instance, the overall impact residue for $S_1$ under selecting subsets $(\{C_1\}, \{C_3\})$ for threats $T_1$ and $T_2$ is as below: 

   $\mathit{ir}_{s_1}^{\mathit{avg}}(C)=\frac{1}{|2|}( ({ir}_{s_{1}}(T_1, \{C_1\})+{ir}_{s_{1}}(T_2, \{C_3\}))$= $\frac{1}{|2|}(0.45+0.225)=0.351$
   
   Under different subset combinations, we may see different impact residue levels. To know which subsets can be selected as solutions, we take advantage of Pareto optimal notation. In the following table, all possible subset combinations and overall impact residues for $S_1$ and $S_2$ are listed: 
   \begin{center}
   \scriptsize
    \begin{tabular}{l|c|c}{\centering}
    &$\mathit{ir}_{s_1}^{\mathit{avg}}(C)$&$\mathit{ir}_{s_2}^{\mathit{avg}}(C)$  \\ \hline\hline
    $((T_1, \{C_1\}), (T_2, \{C_3\}))$ & 0.393       & 0.346          \\ 
    $((T_1, \{C_1\}), (T_2, \{C_4\}))$ & 0.359       & 0.329         \\
    $((T_1, \{C_1\}), (T_2, \{C_5\}))$ & 0.393       & 0.346        \\
    $((T_1, \{C_1\}), (T_2, \{C_3, C_4\}))$ & 0.325   & 0.312         \\
    $((T_1, \{C_1\}), (T_2, \{C_3, C_5\}))$ & 0.359   & 0.329         \\
    $((T_1, \{C_1\}), (T_2, \{C_4, C_5\}))$ & 0.325   & 0.312         \\
    $((T_1, \{C_1\}), (T_2, \{C_3, C_4, C_5\}))$ & 0.313  & 0.302   \\
    $((T_1, \{C_2\}), (T_2, \{C_3\}))$ & 0.318     & 0.259   \\
    $((T_1, \{C_2\}), (T_2, \{C_4\}))$ & 0.284     & 0.242 \\
    $((T_1, \{C_2\}), (T_2, \{C_5\}))$ & 0.318    & 0.259  \\
    $((T_1, \{C_2\}), (T_2, \{C_3, C_4\}))$ & 0.25  & 0.225 \\
    $((T_1, \{C_2\}), (T_2, \{C_3, C_5\}))$ & 0.284   & 0.242  \\
    $((T_1, \{C_2\}), (T_2, \{C_4, C_5\}))$ & 0.25  & 0.225    \\
    $((T_1, \{C_2\}), (T_2, \{C_3, C_4, C_5\}))$ & 0.238 & 0.215 \\
    $((T_1, \{C_1, C_2\}), (T_2, \{C_3\}))$ & 0.243       & 0.171  \\ 
    $((T_1, \{C_1, C_2\}), (T_2, \{C_4\}))$ & 0.209       & 0.154   \\
    $((T_1, \{C_1, C_2\}), (T_2, \{C_5\}))$ & 0.243       & 0.171    \\
    $((T_1, \{C_1, C_2\}), (T_2, \{C_3, C_4\}))$ & 0.175  & 0.137   \\
    $((T_1, \{C_1, C_2\}), (T_2, \{C_3, C_5\}))$ & 0.209  & 0.154 \\
    $((T_1, \{C_1, C_2\}), (T_2, \{C_4, C_5\}))$ & 0.175   & 0.137 \\
    $((T_1, \{C_1, C_2\}), (T_2, \{C_3, C_4, C_5\}))$ & 0.163  & 0.127  \\
    \end{tabular}
    \end{center}
   
\end{Example}


\begin{Example}{}{}
   \small{ 
   To mitigate the risk of $T_1$ and $T_2$ in Example 1, we identify a set of controls. Let imagine
   $\mathbb{P}(\mathcal{C}) =$ \{\emph{$c_1$=Ensuring data minimization, $c_2$=Enabling data deletion, $c_3$=Providing confidential communication, $c_4$=Logging access to personal data, $c_5$=Ensuring data anonymization}\}\ where the first two controls are devoted to $T_1$ and the rest are for $T_2$. Therefore, $m_T:\mathbb{P}(\mathcal{C})\to [0..1)$ is as below:
   \begin{center}
    \scriptsize
    \begin{tabular}[t]{c|c}
                                 $m_{T1}$     &        \\ \hline\hline
                                \{$c_1$\}     & 0.25   \\
                                \{$c_2$\}     & 0.5    \\
                                \{$c_1,c_2$\} & 0.375  
     \end{tabular}                          
    \begin{tabular}[t]{c|c} 
                                $m_{T2}$       &     \\ \hline\hline
                                \{$c_3$\}      & 0.16  \\
                                \{$c_4$\}      & 0.33  \\
                                \{$c_5$\}      & 0.16  \\
                                \{$c_3$, $c_4$\}      & 0.5  \\
                                \{$c_3$, $c_5$\}      & 0.33  \\
                                \{$c_4$, $c_5$\}      & 0.5  \\
                                \{$c_3,c_4,c_5$\}  & 0.66 
    \end{tabular}
    \begin{tabular}[t]{c|c} 
                                $m_{T3}$       &     \\ \hline\hline
                                $\emptyset$      & 0  \\
                                \{$c_5$\}      & 0.16  \\
    \end{tabular}
    \end{center}
    where the first column of each table lists possible subsets and the second provides the assigned mitigation levels for each of these subsets. 
    For instance, the assigned mitigation level for subset (\{$c_1,c_2$\}) to mitigate $T_1$ is $0.375$.
    The impact residue ($i_s(T)\cdot (1-m_T(C))$) for each of these subsets is computed as following: 
    }
    \begin{alignat*}{2}\scriptsize
    \begin{aligned} & \begin{cases}
            {ir}_{s_{1}}(T_1, \{C_1\})= 0.45 & \\
            {ir}_{s_{1}}(T_1, \{C_2\})= 0.3 & \\
            {ir}_{s_{1}}(T_1, \{C_1, C_2\})= 0.15 & \\
            --------- \\
            {ir}_{s_{1}}(T_2, \{C_3\})= 0.336 & \\
            {ir}_{s_{1}}(T_2, \{C_4\})= 0.268 & \\
            {ir}_{s_{1}}(T_2, \{C_5\})= 0.336 & \\
            {ir}_{s_{1}}(T_2, \{C_3, C_4\})= 0.2 & \\
            {ir}_{s_{1}}(T_2, \{C_3, C_5\})= 0.268 & \\
            {ir}_{s_{1}}(T_2, \{C_4, C_5\})= 0.2 & \\
            {ir}_{s_{1}}(T_2, \{c_3,c_4,c_5\})= 0.176 & \\
      \end{cases}\\
      \end{aligned}
      \begin{aligned}
      & \begin{cases}
            {ir}_{s_{2}}(T_1, \{C_1\})= 0.525 & \\
            {ir}_{s_{2}}(T_1, \{C_2\})= 0.35 & \\
            {ir}_{s_{2}}(T_1, \{C_1, C_2\})= 0.175 & \\
            --------- \\
            {ir}_{s_{2}}(T_2, \{C_3\})= 0.168 & \\
            {ir}_{s_{2}}(T_2, \{C_4\})= 0.134 & \\
            {ir}_{s_{2}}(T_2, \{C_5\})= 0.168 & \\
            {ir}_{s_{2}}(T_2, \{C_3, C_4\})= 0.1 & \\
            {ir}_{s_{2}}(T_2, \{C_3, C_5\})= 0.134 & \\
            {ir}_{s_{2}}(T_2, \{C_4, C_5\})= 0.1 & \\
            {ir}_{s_{2}}(T_2, \{c_3,c_4,c_5\})= 0.088 & \\
      \end{cases} \\
      \end{aligned}
    \end{alignat*}
   
   \small{where each value above is derived from the existing subset of controls and the impact levels for each threat.
    }
 \end{Example}
 
 
    % \begin{center}
    % \small
    % \begin{tabular}{llcccc}
    % \multirow{2}{*}{$\mathcal{T}$} & \multirow{2}{*}{$\mathcal{C}$} & \multicolumn{3}{c}{$a_T(C)$}   &  \multirow{2}{*}{$\tilde{X}_T$} \\ \cline{3-5} 
    %                         &   & $N=0$ &$P=0.5$ & $F=1$ & \\ \hline \hline
    % \multirow{2}{*}{$T_1$}  & $C_1$     &\ding{53}&   &  &\multirow{2}{*}{$1-\frac{0+0.5}{|2|}=0.25$}  \\
    %                         & $C_2$     &    &\ding{53}&  &  \\ \hline
    % \multirow{2}{*}{$T_1$}  & $C_3$     &    &\ding{53}&  &\multirow{2}{*}{$1-\frac{0+0.5}{|2|}=0.75$}  \\
    %                         & $C_4$     &    &  &\ding{53}&  \\ \hline
    % $T_3$                   & $C_5$     &    &\ding{53}&  & $1-\frac{0+0.5}{|1|}=0.5$
    % \end{tabular}

    % \end{center}
    
    \begin{Example}{}{} \small
%   So far we learnt from the two previous examples that 
    From Example 2, we learnt how the impact residue for each threat can be computed. Through $\mathit{ir}_s^{\mathit{avg}}(C)=\frac{1}{|\mathcal{T}|} \Sigma_{T\in \mathcal{T}}~ \mathit{ir}_s(T,C)$
    the overall impact residue can be obtained for each stakeholder. 
    % by having the derived impact residue for each subset 
    % would be as follow:
    For instance, the overall impact residue for $S_1$ under selecting subsets $(\{C_1\}, \{C_3\})$ for threats $T_1$ and $T_2$ is as below: 

   $\mathit{ir}_{s_1}^{\mathit{avg}}(C)=\frac{1}{|2|}( ({ir}_{s_{1}}(T_1, \{C_1\})+{ir}_{s_{1}}(T_2, \{C_3\}))$= $\frac{1}{|2|}(0.45+0.225)=0.351$
   
   Under different subset combinations, we may see different impact residue levels. To know which subsets can be selected as solutions, we take advantage of Pareto optimal notation. In the following table, all possible subset combinations and overall impact residues for $S_1$ and $S_2$ are listed: 
   \begin{center}
   \scriptsize
    \begin{tabular}{l|c|c}{\centering}
    &$\mathit{ir}_{s_1}^{\mathit{avg}}(C)$&$\mathit{ir}_{s_2}^{\mathit{avg}}(C)$  \\ \hline\hline
$((T_1, \{C_1\}), (T_2, \{C_3\}), (T_3,\{\emptyset\} ))$ & 0.225& 0.262\\ 
$((T_1, \{C_1\}), (T_2, \{C_4\}), (T_3,\{\emptyset\} ))$ & 0.175& 0.137\\
$((T_1, \{C_1\}), (T_2, \{C_3,C_4\}), (T_3,\{\emptyset\} ))$ & 0.2& 0.2\\
$((T_1, \{C_1\}), (T_2, \{C_3\}), (T_3,\{C_5\} ))$ & 0.2& 0.275\\
$((T_1, \{C_1\}), (T_2, \{C_4\}), (T_3,\{C_5\} ))$ & 0.166& 0.191\\
$((T_1, \{C_1\}), (T_2, \{C_3,C_4\}), (T_3,\{C_5\} ))$ & 0.183& 0.233\\
$((T_1, \{C_2\}), (T_2, \{C_3\}), (T_3,\{\emptyset\} ))$ & 0.337& 0.3\\ 
$((T_1, \{C_2\}), (T_2, \{C_4\}), (T_3,\{\emptyset\} ))$ & 0.287& 0.175\\
$((T_1, \{C_2\}), (T_2, \{C_3,C_4\}), (T_3,\{\emptyset\} ))$ & 0.312& 0.237\\
$((T_1, \{C_2\}), (T_2, \{C_3\}), (T_3,\{C_5\} ))$ & 0.275& 0.3\\
$((T_1, \{C_2\}), (T_2, \{C_4\}), (T_3,\{C_5\} ))$ & 0.241& 0.216\\
$((T_1, \{C_2\}), (T_2, \{C_3,C_4\}), (T_3,\{C_5\} ))$ & 0.258& 0.258\\
$((T_1, \{C_1, C_2\}), (T_2, \{C_3\}), (T_3,\{\emptyset\} ))$ & 0.162& 0.225\\ 
$((T_1, \{C_1, C_2\}), (T_2, \{C_4\}), (T_3,\{\emptyset\} ))$& 0.112&0.1\\
$((T_1, \{C_1, C_2\}), (T_2, \{C_3,C_4\}), (T_3,\{\emptyset\} ))$& 0.137&0.162\\
$((T_1, \{C_1, C_2\}), (T_2, \{C_3\}), (T_3,\{C_5\} ))$ & 0.158& 0.25\\
$((T_1, \{C_1, C_2\}), (T_2, \{C_4\}), (T_3,\{C_5\} ))$ & 0.125& 0.166\\
$((T_1, \{C_1, C_2\}), (T_2, \{C_3,C_4\}), (T_3,\{C_5\} ))$ & 0.141& 0.208\\

    \end{tabular}
    \end{center}
   
\end{Example}

\begin{comment}
the finite set of distinct values obtained by considering all possible assignments to the controls in $C\in\mathbb{P}(\mathcal{C})$ according to $a_T$, i.e.
\begin{equation*}
    X_T = \left\{ 1-\frac{\Sigma_{c\in C} ~ a_T(c)}{|{C}|} | 
    C\subseteq \mathcal{C}\right\} .
\end{equation*}
Interestingly, it is possible to derive solutions for~\eqref{eq:msrmp} from those of~\eqref{eq:msrmp2} as follows.  Let $\langle x_T^*\rangle_{T\in \mathcal{T}}$ a solution for~\eqref{eq:msrmp2}.  By definition, there must exist $C^*\subseteq \mathcal{C}$ such that $x_T^*=1-\frac{\Sigma_{c\in C^*} ~ a_T(c)}{|{C}|}$ for each $T\in \mathcal{T}$.  It is possible to find such $C^*$ (there can be more than one) by enumerating all possible subsets of $\mathcal{C}$; in this way, we can discover all $C^*$ that are solutions of~\eqref{eq:msrmp}.        

For each $T$ in $\mathcal{T}$, $|X_T|$ is the number of distinct sums that can be obtained by adding a value in $\{0,0.5,1\}$ associated to a control in all possible sub-sets of $\mathcal{C}$.  The space of solutions of~\eqref{eq:msrmp2} is thus $\Pi_{T\in \mathcal{T}} |X_{T}|$.  Despite  this number is likely to be less than $3^{|\mathcal{C}|}$, it may still be quite a large number making the solution of~\eqref{eq:msrmp2} difficult.  Fortunately, it is possible to further reduce the search space by exploiting some domain knowledge, namely the fact that certain controls are only meaningful for mitigating the negative effects of certain threats while having no effect on others.  To model this knowledge, we assume that, for each threat $T$ in $\mathcal{T}$, we associate a subset $C_T\subseteq \mathcal{C}$ to $T$, i.e.\ $C_T$ contains those controls whose (possibly combined) adoption can potentially mitigate the threat $T$, i.e.\ $m_T(C_T) \neq 0$, but has no effect on the other threats, i.e.\ $m_T(C_{T'}) = 0$ for $T$ and $T'$ in $\mathcal{T}$ with $T\neq T'$.  As a consequence, we can replace the set $X_T$ in~\eqref{eq:msrmp2} with the following:
\end{comment}

==> Removed/Threat_Modeling.tex <==
\section{Threat Modeling}\label{sec:threat-modeling}
Threat modeling has a vital role in building a secure software system by considering how an adversary might compromise the system.
Indeed, it supports understanding security and privacy threats in a given system, how those threats impact data subjects and the organization as the data controller and identifying possible security and privacy countermeasures to mitigate potential attacks.
It is highly recommended to apply threat modeling early in the development cycle, where potential issues can be detected early and remedied to prevent possible later consequences.
There are several approaches that may be used while undertaking threat modeling, such as Microsoft STRIDE~\cite{shostack2014threat}, PASTA~\cite{ucedavelez2015risk}, LINDDUN~\cite{wuyts2015linddun}, and Trike~\cite{saitta2005trike}. Each threat modeling technique follows a somewhat different set of phases.
Not all methods are comprehensive, or in other words, a particular threat modeling method is not suggested over the others. The decision to select a method depends on the defined project’s needs and specific concerns~\cite{shevchenko2018threat}. Indeed, the best model for your requirements is determined by the kind of threats you are attempting to model and the purpose for which you are doing so.
% However, our methodology’s threat modeling phase is roughly the same as other threat modeling methods in terms of the processes that need to be performed. 
Our objectives of conducting this phase are: (i) to have a comprehensive understanding of the system that supports security and privacy-aware specification of the data processing, (ii) to identify potential threat scenarios, and then (iii) to determine countermeasure controls according to the identified threats. In this phase, the following steps require to be fulfilled:

% Our threat modeling phase is almost the same as other threats modeling in terms of the processes that need to be done, with this objective to have a comprehensive understanding of the system, identifying potential threat scenarios, and determining countermeasure controls. In this phase, the following processes require to be fulfilled:

\subsection{\textbf{Security and privacy-aware specification of the data processing}}
\begin{figure} [!t]
    \centering
	\includegraphics[width=0.95\textwidth]{Figures/DFD_ACME.pdf}
    \caption{High-level data flow diagram in our eHealth scenario.}
    \label{fig:DFD}
\end{figure}

Security by Design (SbD) and Privacy by Design (PbD) are principles increasingly identified as necessary for dealing with design faults that may jeopardize security or privacy in the system~\cite{alshammari2017}. 
Furthermore, their application is also envisaged by the GDPR, as it demands Data Protection by Design (DPbD) for any systems that involve personal data in their processing.

[THIS SECTION NEEDS TO BE EXTENDED AND REFINED]

The first step of threat modeling aims to characterize a system in such a comprehensive and detailed way that potential security and privacy threats can be found. 
In this step, all the assets and the main actors involved in the system must be identified.
For example, Figure~\ref{fig:scenario} depicts the main actors and their interactions with the system's components in our scenario. At the client-side (End-user), the Mobile Health App dynamically receives the biometric data from the smart health device, which is worn/used by the patient. Then the data is transferred to the HCare-web server (Application provider) for further processing. After receiving any updates (such as biometric data or user requests) from the patients, the doctors monitor their health condition at the health service provider side. Through the HCare-web, doctors can write a prescription, respond to requests, initiate a medical alert, etc. 

In this step, the data flow diagram (DFD) aids represent how data flow through the system and handled by different sub-processes. A DFD presents a logical depiction of the system’s implementation and shows the system’s large-scale architecture. It illustrates what entities exist in implementing the system and how these entities exchange information. It is also helpful for the threat identification process to characterize how adversaries can threaten the various phases of the data flow, such as collecting, storing, using, transferring, and deleting.
For our scenario, we decided to use the DFD in Figure~\ref{fig:DFD} as the system documentation in Figure~\ref{fig:methodology}, as this helps highlight how data is modified during the data processing activity under consideration.  

% The data flow diagram of processing the health data recorded in our scenario is depicted in Figure~\ref{fig:DFD}.  

% \subsection{\textbf{Selecting threat types} }

\subsection{\textbf{Threat scenario identification}}
\begin{table}[!b] \center
    \caption{Security and privacy threat types defined in~\cite{shostack2014threat,wuyts2015linddun}}
    \includegraphics[width=0.99\textwidth]{Figures/Threat-types.pdf}
    \label{tab:threat-types}
\end{table}
A threat is a potential adverse action or event facilitated by a vulnerability that results in an undesired impact on the system. Threats usually may come from authorized users (insiders) or unauthorized users (outsiders). All the information gathered from the last phase will assist in identifying possible threats in the system.
Utilizing the provided threat lists will also help in the threat identification process by reviewing each asset, process, access point, and data flow in the system and creating threat scenarios regarding violation of security and privacy properties. 
In general, threats in a given system can be divided into two broad classes, namely security and privacy threat types. 
The identification of security and privacy threats entails knowledge of the types of threats to be identified.
High-level categories of security~\cite{hernan2006threat} or privacy~\cite{deng2011privacy} threats---which might comprise multiple sub-types of threats in a hierarchical structure---are used in threat modeling. Here, the word “categories” is sub-optimal, as it is aimed only to help in the remainder of the main types of threats.
The categories are not disjunct groups under which all the different threat types can be unambiguously placed. Rather, the many forms of threats are overlapping and dependent~\cite{sion2020}. For instance, spoofing an identity can lead to the elevation of privilege in the system. In addition to the threat modeling threat types, there are a variety of different knowledge sources on security and privacy concerns at various abstraction levels. Low-level vulnerabilities in concrete software products~\cite{cve}, design flaws~\cite{arce2014,hosseini2017,tuma2019}, architectural weakness~\cite{cwe, santos2017catalog}, and attack patterns~\cite{CAPEC} are only a few examples in this regard.

~STRIDE is a well-established threat modeling presented by Microsoft to identify security threat types. 
It is an acronym for \emph{Spoofing, Tampering, Repudiation, Information Disclosure, Denial of Service, }and \emph{Elevation of privilege}. These threats are the opposite of the primary security properties: authentication, integrity, non-repudiation, confidentiality, availability, and authorization. 
LINDDUN is another well-known threat modeling to identify privacy threats in the system, and it stands for \emph{Linkability, Identifiability, Non-repudiation, Unawareness, Detectability, Disclosure of information,} and \emph{Non-compliance}. 
These threats are the negation of privacy properties: unlinkability, anonymity and pseudonymity, plausible deniability, undetectability and unobservability, confidentiality, content awareness, policy and consent compliance. All the mentioned threats above are described in Table~\ref{tab:threat-types}. Notice that the \emph{disclosure information} is a common threat in both methods. Therefore, we do not describe it again for LINDDUN in Table~\ref{tab:threat-types}. Indeed, Table~\ref{tab:threat-types} is the content of the database in Figure~\ref{fig:methodology} called Security $\&$ Privacy threat types. It is possible to customize it depending on the scenario considered, and here, we use this for our scenario.

\begin{table}[!b] \center
    \caption{An example of possible threat scenarios and their mapped threat types in the ACME scenario}
    \includegraphics[width=0.99\textwidth]{Figures/Threat-scenarios.pdf}
    \label{tab:threat-table}
\end{table}


Each security and privacy property can be threatened by different type of threats in a given system. 
% Therefore, in this step, the potential threat scenarios must be identified. 
For the sake of simplicity, Table~\ref{tab:threat-table} shows five possible threat scenarios relevant to our scenario. This is the list of threat scenarios as derived by the threat scenario identification process in Figure~\ref{fig:methodology}, by using the database of Security $\&$ Privacy threat types (Table~\ref{tab:threat-types}) together with the system documentation in Figure~\ref{fig:methodology}, i.e., the DFD in Figure~\ref{fig:DFD}.
% Each threat is mapped to one (or more) possible threat type(s), as well as the relevant data processing principles (we will explain these principles in Section~\ref{sec:threat-principle}) taken from those listed in the GDPR and relevant approaches such as STRIDE and LINDDUN.


\subsection{\textbf{Determining security and privacy controls}}
Security and privacy controls are the administrative, technical, and physical safeguards or countermeasures to avoid, detect, counteract, or mitigate security and privacy risks within an organization~\cite{ref_35,force2018risk}.
To establish and extract the required controls inside a system, there are several frameworks, guidelines, and best practices.
For example, NIST Special Publication 800-53~\cite{draft2017security} on Security and Privacy Controls for Information Systems and Organizations is the specification of privacy and security controls for public offices in the United States. 
It includes a wide collection of predefined controls, as well as appendices that demonstrate how to select controls that respond to different risk and effect levels.

The last step of our threat modeling phase is to determine the security and privacy controls for each identified threat scenarios. 
% In our scenario, we have determined the security and privacy controls for each threat, in total twenty-five controls for five identified threat scenarios. 
We have determined and listed the security and privacy controls in our scenario. 
For instance, for the \emph{unlimited data storage} threat (T1) in Table~\ref{tab:threat-table}, we associate some possible controls such as \emph{the purpose specification, ensuring limited data processing, ensuring data minimization}, and \emph{implementing data deletion mechanisms}. 
While for the \emph{Denial of Service} threat (T4), possible associated controls can be \emph{enabling offline authentication, network monitoring}, and \emph{implementing the preventing DoS attack mechanisms like firewalls, IDS, etc}. The complete association is provided later in Table~\ref{tab:threat-control}. 

% However, due to avoid multi-time representing them, and since we need to refer to these controls in the \emph{Risk Calculation and Optimization} phase (cf. Section~\ref{sec:optimization}), therefore, we will present them all together with the threat scenarios in Table~\ref{tab:threat-control}.


